Optimization for Supervised Machine Learning: Randomized Algorithms for Data and Parameters

Many key problems in machine learning and data science are routinely modeled as optimization problems and solved via optimization algorithms. With the increase of the volume of data and the size and complexity of the statistical models used to formulate these often ill-conditioned optimization tasks, there is a need for new efficient algorithms able to cope with these challenges. In this thesis, we deal with each of these sources of difficulty in a different way. To efficiently address the big data issue, we develop new methods which in each iteration examine a small random subset of the training data only. To handle the big model issue, we develop methods which in each iteration update a random subset of the model parameters only. Finally, to deal with ill-conditioned problems, we devise methods that incorporate either higher-order information or Nesterov's acceleration/momentum. In all cases, randomness is viewed as a powerful algorithmic tool that we tune, both in theory and in experiments, to achieve the best results. Our algorithms have their primary application in training supervised machine learning models via regularized empirical risk minimization, which is the dominant paradigm for training such models. However, due to their generality, our methods can be applied in many other fields, including but not limited to data science, engineering, scientific computing, and statistics.

==> ACD/sec-experiments.tex <==
\section{Experiments} \label{sec:exp}

We perform extensive numerical experiments to justify that minibatch \texttt{ACD} with importance sampling works well in practice. Here we present a few selected experiment only; more can be found in Appendix~\ref{sec:extra_exp}. 

In most of plots we compare of both accelerated and non-accelerated \texttt{CD} with all samplings $S_1,S_2,S_3$ introduced in Sections~\ref{sec:sam1}, \ref{sec:sam2} and \ref{sec:sam3} respectively. We refer to \texttt{ACD} with sampling $S_3$ as \texttt{AN} (\texttt{A}ccelerated \texttt{N}onuniform), \texttt{ACD} with sampling $S_1$ as \texttt{AU}, \texttt{ACD} with sampling $S_2$ as \texttt{AN2}, \texttt{CD} with sampling $S_3$ as \texttt{NN}, \texttt{CD} with sampling $S_1$as \texttt{NU} and \texttt{CD} with sampling $S_2$ as \texttt{NN2}. We compare the methods for various choices of the expected minibatch sizes $\tau$ and on several problems. 

 
In Figure~\ref{fig:logreg_big}, we report on a logistic regression problem with a few selected LibSVM~\cite{chang2011libsvm} datasets.  For larger datasets, pre-computing both strong convexity parameter $\sigma$ and  $v$ may be expensive (however, recall that for $v$ we need to tune only one scalar). Therefore, we choose ESO parameters $v$ from Lemma~\ref{thm:special-ESO-result}, while estimating the smoothness matrix as $10\times$ its diagonal. An estimate of the strong convexity $\sigma$ for acceleration was chosen to be the minimal diagonal element of the smoothness matrix. We provide a formal formulation of the logistic regression problem, along with  more experiments applied to further datasets in Appendix~\ref{exp:logreg}, where we choose $v$ and $\sigma$ in full accord with the theory.

\begin{figure}[t]
\centering
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_1_data_rcv.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_8_data_rcv.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_64_data_rcv.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_512_data_rcv.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_1_data_rea.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_8_data_rea.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_64_data_rea.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_512_data_rea.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_1_data_new.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_8_data_new.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_64_data_new.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{NEW99_REMOTE_tau_512_data_new.png}
        %\caption{ Residual vs. iteration  }\label{fig:bl_ex_flops}
\end{minipage}%
\caption{Six variants of coordinate descent (\texttt{AN}, \texttt{AU}, \texttt{NN}, \texttt{NU}, \texttt{AN2} and \texttt{AU2})  applied to a logistic regression problem, with minibatch sizes $\tau=1, 8, 64$ and $512$.}\label{fig:logreg_big}
\end{figure}

Coordinate descent methods which allow for separable proximal operator were proven to be efficient to solve ERM problem, when applied on dual~\cite{shalev2011stochastic,SDCA,shalev2014accelerated,zhao2015stochastic}.
Although we do not develop proximal methods in this paper, we empirically demonstrate that \texttt{ACD} allows for this extension as well. As a specific problem to solve, we choose dual of SVM with hinge loss. The results and a detailed description of the experiment are presented in Appendix~\ref{sec:SVM}, and are indeed in favour of \texttt{ACD} with importance sampling. Therefore, \texttt{ACD} is not only suitable for \emph{big dimensional} problems, it can handle the \emph{big data} setting as well.

Finally, in Appendix~\ref{sec:artif} we present several synthetic examples in order to shed more light on  acceleration and importance sampling, and to see how its performance depends on the  data. We also study how minibatch size influences the convergence rate. All the experimental results clearly show that  acceleration, importance sampling and minibatching have a significant impact on practical performance of \texttt{CD} methods. Moreover, the difference in the performance of samplings $S_2$ and $S_3$ is negligible, and therefore we recommend using $S_3$, as it is not limited by the bound on expected minibatch sice $\tau$



==> local.tex <==
\chapter{Federated Learning of a Mixture of Global and Local Models}

\label{local}


\graphicspath{{local/plots/}}




With the proliferation of mobile phones, wearable devices, tablets, and smart home devices comes an increase in the volume of data captured and stored on them. This data contains a wealth of potentially useful information to the owners of these devices, and more so if appropriate machine learning models could be trained on the heterogeneous data stored across the network of such devices.  The traditional approach involves moving the relevant data to a  data center where centralized machine learning techniques can be efficiently applied~\cite{Dean2012, AIDE}.  However, this approach is not without issues.  First, many device users are increasingly sensitive to privacy concerns and prefer their data to never leave their devices. Second, moving data from their place of origin to a centralized location is very inefficient in terms of energy and time. 

\section{Federated learning}

{\em Federated learning (\acrshort{FL})} \cite{FedAvg2016, FEDLEARN,   FEDOPT, FL2017-AISTATS} has emerged as an interdisciplinary  field focused on addressing these issues by training machine learning models directly on  edge devices.  The currently prevalent paradigm~\cite{FL_survey_2019, FL-big} casts supervised FL as an empirical risk minimization problem of the form
\begin{equation}\label{eq:local_ERM-traditional}  
\min \limits_{x\in \R^d} \frac{1}{n}\sum \limits_{i=1}^n f_i(x),
\end{equation}
where $n$ is the number of devices participating in training, $x\in \R^d$ encodes the $d$ parameters of  a {\em global model}  (e.g., weights of a neural network) and $f_i(x)\eqdef \EE_{\xi\sim \cD_i}{f(x,\xi)}$ represents the aggregate loss of model $x$ on the local data represented by distribution $\cD_i$ stored on device $i$. One of the defining characteristics of FL is that the data distributions $\cD_i$ may possess very different properties across the devices. Hence, any potential FL method  is explicitly required to be able to work under the {\em heterogeneous} data setting.


The most popular method for solving \eqref{eq:local_ERM-traditional} in the context of FL is the FedAvg algorithm~\cite{FedAvg2016}. In its most simple form, when one does not employ partial participation, model compression, or stochastic approximation, FedAvg reduces to Local Gradient Descent ({\tt LGD})~\cite{localGD, localSGD-AISTATS2020}, which is an extension of {\tt GD} performing more than a single gradient step on each device before aggregation.  FedAvg has been shown to work well empirically, particularly for non-convex problems, but comes without convergence guarantees and can diverge in practical settings when data are heterogeneous.


\subsection{Some issues with current approaches to FL}

%Variance reduced local {\tt SGD}: \cite{karimireddy2019scaffold, liang2019variance} (both do local {\tt SGD} with a shift which under some assumptions improves the rate)
%
%Variance reduced local {\tt SGD} robust to Byzantine attacks: \cite{wu2019federated}


The first motivation for our research comes from the appreciation that data heterogeneity does not merely present challenges to the design of new provably efficient training  methods for solving  \eqref{eq:local_ERM-traditional}, but {\em also inevitably raises questions about the utility of such a global solution to individual users.} Indeed, a global model trained across all the data from all devices might be so removed from the typical data and usage patterns experienced by an individual user as to render it virtually useless. This issue has been observed before, and various approaches have been proposed to address it. For instance, the MOCHA \cite{NIPS2017_FL-multitask} framework uses a multi-task learning approach to allow for personalization. A generic online algorithm for gradient-based parameter-transfer meta-learning \cite{Khodak2019FLmeta} was demonstrated to improve practical performance over FedAvg~\cite{FL2017-AISTATS}. Approaches based on variational inference~\cite{FL2019variational}, cyclic patterns in practical FL data sampling  \cite{Eichner2019semi-cyclicSGD_for_FL} and transfer learning \cite{Zhao2018FL-transfer-learn} have been proposed.

The second motivation for our work is the realization that even very simple variants of FedAvg, such as {\tt LGD}, which should be easier to analyze, fail to provide theoretical improvements in communication complexity over their non-local cousins, in this case, {\tt GD} \cite{localGD, localSGD-AISTATS2020}.  This observation is at odds with the practical success of local methods in FL. This leads us to ask the question: 
\begin{quote}{\em If {\tt LGD} does not theoretically improve upon {\tt GD} as a solver for the traditional global problem~\eqref{eq:local_ERM-traditional}, perhaps  {\tt LGD} should not be seen as a method for solving~\eqref{eq:local_ERM-traditional} at all. In such a case, what problem does {\tt LGD} solve?}
\end{quote}

 A good answer to this question would shed light on the workings of {\tt LGD}, and by analogy, on the role local steps play in more elaborate  FL methods such as local {\tt SGD}~\cite{localSGD-Stich, localSGD-AISTATS2020} and FedAvg. 


\section{Contributions \label{sec:local_contrib}}

In our work we argue that the two motivations mentioned in the introduction  point in the same direction, i.e., we show that {\em a single solution can be devised addressing both problems at the same time.} 

Our main contributions are:

\begin{itemize}
\item  {\bf New formulation of FL which seeks a mixture of  global and local models.} We propose a {\em new optimization formulation of FL.}  Instead of learning a single global model by solving \eqref{eq:local_ERM-traditional}, we propose to learn a mixture of the global model and the purely local models which can be trained by each device $i$ on its own, using its data $\cD_i$ only.  Our formulation (see \eqref{eq:local_main}  in Section~\ref{sec:local_new_formulation}) lifts the problem from $\R^d$ to $\R^{nd}$, allowing each device $i$ to learn a personalized model $x_i\in \R^d$. However, these personalized models are explicitly encouraged to not depart too much from their mean by the inclusion of a quadratic penalty $\Phi$ multiplied by a penalty parameter $\lambda\geq 0$.\footnote{The idea of softly-enforced similarity of the local models was already introduced in the domain of decentralized optimization~\cite{lan2018communication, gorbunov2019optimal}. However, their motivation is vastly different to ours (besides not considering FL or local algorithms) -- the mentioned methods still aim to find the global model by having the penalty parameter inversely proportional to the target accuracy $\varepsilon$.}

\item  {\bf Theoretical properties of the new formulation.} We study the properties of the optimal solution of our formulation, thus developing an algorithmic-free theory. When the penalty parameter is set to zero, then obviously, each device is allowed to train their own model without any dependence on the data stored on other devices. Such purely local models are rarely useful. We prove that the optimal local models converge to the traditional global model characterized by \eqref{eq:local_ERM-traditional} at the rate $\cO(1/\lambda)$. We also show that the total loss evaluated at the local models is always not higher than the total loss evaluated at the global model (see Theorem~\ref{thm:local_penalty}).  Moreover, we prove an insightful structural result for the optimal local models: the optimal model learned by device $i$ arises by subtracting the gradient of the loss function stored on that device evaluated at the same point (i.e., a local model) from the average of the optimal local models (see Theorem~\ref{thm:local_characterization}).  As a byproduct, this theoretical result sheds new light on the key update step in the model agnostic meta-learning (MAML) method \cite{MAML2017}, which has a similar but subtly different structure. The subtle difference is that the MAML update obtains the local model by subtracting the gradient evaluated at the {\em global} model. While MAML is a heuristic, we provide rigorous theoretical guarantees.

\item  {\bf Loopless {\tt LGD}: non-uniform {\tt SGD} applied to our formulation.} We then propose a randomized gradient-based method---{\em Loopless Local Gradient Descent ({\acrshort{L2GD}})}---for solving our new formulation (Algorithm~\ref{alg:local_L2GD}). This method is, in fact, a non-standard application of {\tt SGD} to our problem, and can be seen as an instance of {\tt SGD} with non-uniform sampling applied to the problem of minimizing the sum of two convex functions~\cite{iprox-sdca, pmlr-v97-qian19b}: the average loss, and the penalty. When the loss function is selected by the randomness in our {\tt SGD} method, the resultant stochastic gradient step can be {\em interpreted} as the execution of a single local {\tt GD} step on each device. Since we set the probability of the loss being sampled to be high, this step is typically repeated multiple times, and this has the effect of taking multiple local {\tt GD} steps. In contrast to standard {\tt LGD}, the number of local steps is not fixed, but random, and follows a geometric distribution. This mechanism is similar in spirit to how the recently proposed loopless variants of {\tt SVRG} \cite{hofmann2015variance, kovalev2019don} work in comparison with the original {\tt SVRG}~\cite{svrg, proxsvrg}. Once the penalty is sampled by our method, the resultant {\tt SGD} step can be interpreted as the execution of an aggregation step. In contrast with standard aggregation, which performs full averaging of the local models, our method is more sophisticated and merely takes a {\em step towards averaging}. However, the step is relatively large. This suggests that perhaps full averaging in modern FL methods such as FedAvg or {\tt LGD} and {\acrshort{LSGD}} is too aggressive, and should be re-examined. 


\item {\bf Convergence theory.} By adapting the general theory from \cite{pmlr-v97-qian19b} to our setting, we obtain theoretical convergence guarantees assuming that each $f_i$ is $L$-smooth and $\mu$-strongly convex (see Theorem~\ref{thm:local_local_gd}). Interestingly, by optimizing  the sampling probability (we get $p^* = \frac{\lambda}{\lambda + L}$) which is an  indirect way of fixing the {\em expected number of local steps} to $1+\frac{L}{\lambda}$, we prove the communication complexity result (i.e., bound on the expected number of communication rounds; see Corollary~\ref{cor:local_optimalp})  \[\frac{2 \lambda }{\lambda + L} \frac{L}{\mu}\log \frac{1}{\varepsilon}.\] We believe that this is remarkable in several ways.  By choosing $\lambda$ small, we tilt our goal towards pure local models, and the number of communication rounds is very small, tending to 0 as $\lambda\to 0$. If $\lambda\to \infty$, our the solution to our formulation converges to the optimal global model,  and {\tt L2GD} obtains the communication bound  $\cO\left(\frac{L}{\mu} \log \frac{1}{\varepsilon}\right)$, which matches the efficiency of {\tt GD}.   Our results can be extended to convex and non-convex regimes, but we do not explore such generalizations here.

\item  {\bf Generalizations: partial participation, local {\tt SGD} and variance reduction.} We further generalize and improve our method and convergence results by allowing for 
\begin{itemize}
\item[(i)] stochastic {\em partial participation} of devices in each communication round,
\item[(ii)]  {\em subsampling} on each device which means we can perform local {\tt SGD} steps instead of local {\tt GD} steps, and  
\item[(iii)]  {\em total variance reduction mechanism} to tackle the variance  coming from three sources: locality of the updates induced by non-uniform sampling (already present in {\tt L2GD}), partial participation and subsampling from local data.
\end{itemize}

Due to its level of generality, this method, which we call {\tt L2SGD++}, is presented in the Appendix only, alongside the associated complexity results.  In the main body of this chapter, we instead present a simplified version thereof, one that does not include partial participation. We call this method {\tt L2SGD+} (Algorithm~\ref{alg:local_L2SGD}). The convergence theory for it is presented in 
Theorem~\ref{thm:local_saga_simple} and Corollary~\ref{cor:local_lsd_optimal_p}.

\item  {\bf Allowing for heterogeneous data.} All our methods and convergence results allow for fully heterogeneous data and do not depend on any assumptions on data similarity across the devices.

\item  {\bf Superior empirical performance.}
We show through ample numerical experiments that our theoretical predictions can be observed in practice.

\end{itemize}

\section{New formulation of FL} \label{sec:local_new_formulation}



% seeking an explicit trade-off between the (traditional) {\em global model}  defined as the solution of \eqref{eq:local_main} and the {\em purely local models} $ \arg \min f_i$, which can be learned by each device $i$ from its own private data  $\cD_i$ without any communication. 

% Instead of learning a single shared {\em global model} $x\in \R^d$, we allow each device $i$ to learn a {\em customized model} $x_i\in \R^d$. These models are allowed to be different but not arbitrarily different. 
% In particular, we introduce a coupling penalty $\Phi$, which encourages the models to be similar.


 We now introduce our new formulation for training supervised FL models:
\begin{equation}\label{eq:local_main}
\begin{aligned}
\min_{x_1,\dots,x_n\in \R^d} &\left\{ F(x) \eqdef f(x) + \lambda \Phi(x) \right\}\\
  f(x) \eqdef  \frac{1}{n}\sum \limits_{i=1}^n  f_i(&x_i), \quad   \Phi(x) \eqdef \frac{1}{2 n}\sum \limits_{i=1}^n \norm{x_i-\bar{x}}^2,
\end{aligned}
\end{equation}
where $\lambda \geq 0 $ is a  penalty parameter,  $x_1,\dots,x_n \in \R^d$ are local models, $x\eqdef (x_1,x_2,\dots,x_n) \in \R^{nd}$ and  $\bar{x}\eqdef \frac{1}{n}\sum_{i=1}^n x_i$ is the average of the local models. 

Due to the assumptions on $f_i$ we will make in Section~\ref{bd798gsd}, $F$ is strongly convex and hence \eqref{eq:local_main} has a unique solution, which we denote $$x(\lambda) \eqdef (x_1(\lambda),\dots,x_n(\lambda)) \in \R^{nd}.$$ We further let $$\bar{x}(\lambda) \eqdef \frac{1}{n}\sum_{i=1}^n x_i(\lambda).$$ 
We now comment on the rationale behind the new formulation.

\paragraph{\bf Local models ($\lambda=0$).} Note that  for each $i$, $x_i(0)$ solves the {\em local problem}
\[ \min_{x_i \in \R^d} f_i(x_i).\]
That is,  $x_i(0)$ is the local model based on data $\cD_i$ stored on device $i$ only. This model can be computed by device $i$ without any communication whatsoever. Typically, $\cD_i$ is not rich enough for this local model to be useful. In order to learn a better model, one has to take into account the date from other clients as well. This, however, requires communication.

\paragraph{\bf Mixed models ($\lambda \in (0,\infty)$).} As $\lambda$ increases, the penalty $\lambda \Phi(x)$ has an increasingly more substantial effect, and communication is needed to ensure that the models are not too dissimilar, as otherwise $\Phi$ would be too large. 

\paragraph{\bf Global model ($\lambda = \infty$).} Let us now look at the limit case $\lambda \to \infty$. Intuitively, this limit case should force the optimal local models to be mutually identical, while minimizing the loss $f$. In particular, this limit case will solve\footnote{If $\lambda=\infty$ and $x_1=x_2=\dots=x_n$ does not hold, we have $F(x)=\infty$. Therefore, we can restrict ourselves on set $x_1=x_2=\dots=x_n$ without loss of generality. }
\[ \min_{x_1,\dots,x_n\in \R^{d}} \left\{ f(x)  \;:\; x_1=x_2=\dots=x_n \right\},\]
which is equivalent to the global formulation \eqref{eq:local_main}.  Because of this, let us defined $x_i(\infty)$ for each $i$ to be the optimal global solution of \eqref{eq:local_ERM-traditional}, and let $x(\infty) \eqdef (x_1(\infty),\dots,x_n(\infty))$. 

\subsection{Technical preliminaries}\label{bd798gsd}
Similarly to the rest of the thesis, we make the following assumption on the functions $f_i$:
\begin{assumption}\label{as:local_smooth_sc_main}
For each $i$, the function $f_i:\R^d\to \R$ is $L$-smooth and $\mu$-strongly convex.
\end{assumption}

Note that the separable structure of $f$ implies that $\left(\nabla f(x)\right)_i = \frac{1}{n}\nabla f_i (x_i)$, i.e., 
\begin{equation}\label{eq:local_nabla f}\nabla f(x) = \frac{1}{n} ( \nabla f_1 (x_1), \nabla f_2 (x_2), \dots,   \nabla f_n (x_n)).\end{equation}   Hence,
 the norm of $\nabla f(x)\in \R^{nd}$ decomposes as
$ \norm{\nabla f(x)}^2 = \frac1n \sum \limits_{i=1}^n \norm{\nabla f_i (x_i)}^2.$

Note that Assumption~\ref{as:local_smooth_sc_main} implies that $f$ is $L_f$-smooth with $L_f \eqdef \frac{L}{n}$ and $\mu_f$-strongly convex with $\mu_f \eqdef \frac{\mu}{n}$. Clearly, $\Phi$ is convex by construction. It can be shown that $\Phi$ is $L_{\Phi}$-smooth with $L_{\Phi}=\frac1n$ (see Appendix). 
% In the limit case $\lambda\to \infty$, all solutions $x_i^*(+\infty)$ become equal. Indeed, they solve  \[x_i^*(+\infty) = \arg\min_z \frac{1}{n}\sum_{i=1}^n f_i(z), \qquad i=1,2,\dots,n.\]
 We can also easily see that 
\begin{equation} \label{eq:local_nhid8gf8f}
\left(\nabla \Phi(x)\right)_i = \frac1n(x_i - \bar{x})
\end{equation} 
(see Appendix), which implies
$$  \Phi(x)   \overset{\eqref{eq:local_main}+\eqref{eq:local_nhid8gf8f}}{=} \frac{n}{2}\sum \limits_{i=1}^n \norm{ (\nabla \Phi(x))_i}^2 = \frac{n}{2} \norm{\nabla \Phi(x)}^2.$$




\subsection{Characterization of optimal solutions}

Our first result describes the behavior of $f(x(\lambda))$ and $\Phi(x(\lambda))$ as a function of $\lambda$.

\begin{theorem} \label{thm:local_penalty}
The function $\lambda \to \Phi(x(\lambda))$ is non-increasing, and
for all $\lambda>0$ we have
\begin{equation} \label{eq:local_dissimilarity} \Phi(x(\lambda)) \leq \frac{f(x(\infty)) - f(x(0))}{\lambda}. \end{equation}
Moreover, the function $\lambda \to f(x(\lambda))$ is non-decreasing, and for all $\lambda \geq 0$ we have
\begin{equation} \label{eq:local_bifg9dd8} f(x(\lambda)) \leq f(x(\infty)).\end{equation}
\end{theorem}

Inequality~\eqref{eq:local_dissimilarity} says that the penalty decreases to zero as $\lambda$ grows, and hence the optimal local models $x_i(\lambda)$ are increasingly similar as $\lambda$ grows. The second statement suggest that the loss $f(x(\lambda))$ increases with $\lambda$, but never exceeds the optimal global loss $f(x(\infty))$ of the standard FL formulation \eqref{eq:local_ERM-traditional}.


We now characterize the optimal local models which connect our model to the MAML framework~\cite{MAML2017}, as mentioned in the introduction.
\begin{theorem} \label{thm:local_characterization}
For each $\lambda >0$ and $1\leq i \leq n$ we have
\begin{equation}\label{eq:local_step_from_mean}
x_i(\lambda) =  \overline{x}(\lambda) - \frac{1}{\lambda }\nabla f_i(x_i(\lambda)).
\end{equation}
Further, we have $ \sum \limits_{i=1}^n \nabla f_i(x_i(\lambda)) = 0$
and $ \Phi(x(\lambda)) = \frac{1}{2 \lambda^2  } \norm{\nabla f(x(\lambda))}^2$.
\end{theorem}
The optimal local models $\eqref{eq:local_step_from_mean}$ are obtained from the average model by subtracting a multiple of the local gradient. Moreover,  observe that the local gradients always sum up to zero at optimality. This is obviously true for $\lambda=\infty$, but it is a bit less obvious that this holds for any $\lambda>0$.


\section{The {\tt L2GD} algorithm} \label{sec:local_L2GD}

In this section we  describe a new randomized gradient-type method for solving our new formulation \eqref{eq:local_main}.  Our method is a non-uniform {\tt SGD} for \eqref{eq:local_main} seen as a 2-sum problem, sampling either  $\nabla f$ or $\nabla \Phi$ to estimate $\nabla F$. Letting $0<p<1$,  we define a stochastic gradient of $F$ at  $x \in \R^{nd}$ as follows
\begin{equation}\label{eq:local_g(x)}g(x) \eqdef \begin{cases} \frac{\nabla f(x)}{1-p} & \text{with probability} \quad 1-p\\
 \frac{\lambda \nabla \Phi(x)}{p} & \text{with probability} \quad p
\end{cases}.\end{equation}

Since $$\E{g(x)} =(1-p) \frac{\nabla f(x)}{1-p} +  p \frac{\lambda \nabla \Phi(x)}{p} = \nabla F(x),$$ the vector $g(x)$ is an unbiased estimator of $\nabla F(x)$. This leads to the following method for minimizing $F$, which we call {\tt L2GD}:
\begin{equation} \label{eq:local_SGD}x^{k+1} = x^k -\alpha G(x^k).\end{equation}
Plugging formulas \eqref{eq:local_nabla f} and \eqref{eq:local_nhid8gf8f} for $\nabla f(x)$ and $\nabla \Phi(x)$ into \eqref{eq:local_g(x)} and subsequently into \eqref{eq:local_SGD}, and writing the resulting method in a distributed manner, we arrive at Algorithm~\ref{alg:local_L2GD}. In each iteration, a coin $\xi$ is tossed and lands $1$  with probability $p$ and $0$ with probability $1-p$. If $\xi=0$, all {\color{red}Devices} perform one local {\tt GD} step \eqref{eq:local_damkpdaosdaon}, and if $\xi=1$, {\color{blue}Master} shifts each local model towards the average via \eqref{eq:local_buiufg98fb}.  As we shall see in Section~\ref{sec:local_analysis}, our convergence theory  limits the value of the stepsize $\alpha$, which has the effect that the ratio $\frac{\alpha \lambda}{n p}$ cannot exceed $\frac{1}{2}$. Hence, \eqref{eq:local_buiufg98fb} is a convex combination of $x_i^k$ and $\bar{x}^k$, which justifies the statement we have made above: $x_i^{k+1}$ shifts towards $\bar{x}^k$ along the line joining these two points.

\begin{algorithm}[h]
  \caption{{\tt L2GD}: Looples Local Gradient Descent}
  \label{alg:local_L2GD}
\begin{algorithmic}
\State{\bfseries Input: }{$x^0_1 = \dots = x_{n}^0\in\R^{d}$, stepsize $\alpha$, probability $p$ }
  \For{$k=0,1,2,\dotsc$}
  \State $\xi = 1$ with probability $p$ and $0$ with probability $1-p$ 
  \If {$\xi=0$}
     \State All {\color{red}Devices} $i=1,\dots,n$ perform a local {\tt GD} step:

        \begin{equation} \label{eq:local_damkpdaosdaon}
        x^{k+1}_i  =x^k_i - \frac{\alpha}{n(1-p)} \nabla f_i(x_i^k)
\end{equation}   
%{\color{blue}Master}  sends model $x_i^{k+1}$ to {\color{red}Device} $i$ for all $i$
  \Else
%  \State All {\color{red}Devices} send their  model  $x_i^k$ to the {\color{blue}Master}
  \State {\color{blue}Master} computes the average $\bar{x}^k = \frac{1}{n}\sum_{i=1}^n x_i^k$
  \State {\color{blue}Master}  for each $i$ computes step towards aggregation
\State 
 \begin{flalign}
 		x^{k+1}_i  = \left(1-\frac{\alpha \lambda}{np}\right) x^k_i + \frac{\alpha \lambda}{np} \bar{x}^k  \label{eq:local_buiufg98fb}
 		\end{flalign}     
  \EndIf
  \EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Understanding communication}

\begin{example} In order to better understand when communication takes place  in Algorithm~\ref{alg:local_L2GD}, consider the following possible sequence of coin tosses: 
$0, 0, 1, 0, 1, 1, 1, 0.$
The first two coin tosses lead to two local {\acrshort{GD}} steps \eqref{eq:local_damkpdaosdaon} on all devices. The third coin toss lands $1$, at which point all local models $x_i^k$ are communicated to the master, averaged to form $\bar{x}^k$, and the step \eqref{eq:local_buiufg98fb} towards averaging is taken. The fourth coin toss is $0$, and at this point, the master communicates the updated local models back to the devices, which subsequently perform a single local {\tt GD} step \eqref{eq:local_damkpdaosdaon}. Then come three consecutive coin tosses landing $1$, which means that the local models are again communicated to the master, which performs three averaging steps  \eqref{eq:local_buiufg98fb}. Finally, the eight coin toss lands $0$, which makes the master send the updated local models back to the devices, which subsequently perform a single local {\tt GD} step.
\end{example}

This example illustrates that communication needs to take place whenever two consecutive coin tosses land a different value. If $0$ is followed by a $1$, all devices communicate to the master, and if $1$ is followed by a $0$, the master communicates back to the devices. It is standard to count each pair of communications, {\color{red}Device}$\to${\color{blue}Master} and the subsequent {\color{blue}Master}$\to${\color{red}Device}, as a single communication round. 

\begin{lemma} \label{lem:local_exp_no_comm}The expected number of communication rounds in $k$ iterations of {\tt L2GD} is $p(1-p)k$.
\end{lemma}



\subsection{The dynamics of local {\tt GD} and averaging steps}

Further, notice that  {\em the average of the local models does not change} during an aggregation step. Indeed, $\bar{x}^{k+1}$ is equal to
\[  \frac{1}{n} \sum \limits_{i=1}^n x_i^{k+1}   \overset{\eqref{eq:local_buiufg98fb}}{=}   \frac{1}{n} \sum \limits_{i=1}^n  \left[\left(1-\frac{\alpha \lambda}{np}\right) x^k_i + \frac{\alpha \lambda}{np} \bar{x}^k \right] = \bar{x}^k.\]

If several averaging steps take place in a sequence, the point $a=\bar{x}^k$ in \eqref{eq:local_buiufg98fb} remains unchanged, and each local model $x_i^k$ merely moves along the line joining the initial value of the local model at the start of the sequence and  $a$, with each step pushing $x_i^k$ closer to the average $a$. 

{\em In summary, the more local {\tt GD} steps are taken, the closer the local models get to the pure local models, and the more averaging steps are taken, the closer the local models get to their average value. The relative number of local {\tt GD} vs. averaging steps is controlled by the parameter $p$: the expected number of local {\tt GD} steps is $\frac{1}{p}$, and the expected number of consecutive aggregation steps is $\frac{1}{1-p}$.}

% \begin{remark}As presented, this method requires a global clock governing the coin toss. In practice one can simply fix the number of local {\tt GD} steps to its expected value $\frac{1}{p}$.\end{remark}

\subsection{Convergence theory }\label{sec:local_analysis}

We fist show that our gradient estimator $g(x)$ satisfies the expected smoothness property \cite{jacsketch, pmlr-v97-qian19b}.


\begin{lemma} \label{lem:local_exp_smoothnes-basic}
Let $\cL\eqdef \frac1n \max\left\{\frac{L}{1-p}, \frac{\lambda }{p}\right\}$ and \[\sigma^2 \eqdef  \frac{1}{n^2}  \sum_{i=1}^n \left( \frac{1}{1-p} \| \nabla f_i(x_i(\lambda))\|^2 + \frac{\lambda^2}{p} \|x_i(\lambda) - \overline{x}(\lambda) \|^2 \right).\] Then for all $x\in \R^d$ we have the inequalities
$$\E{ \norm{g(x) - G(x(\lambda))}^2}  \leq 2\cL \left(F(x)-F(x(\lambda))\right)$$ and
$$\E{\norm{g(x)}^2}  \leq 4 \cL  (F(x)-F(x(\lambda))) + 2 \sigma^2.$$
\end{lemma}



We now present our convergence result for {\tt L2GD}.


\begin{theorem}\label{thm:local_local_gd} Let Assumption~\ref{as:local_smooth_sc_main} hold.
If $\alpha \leq \frac{1}{2\cL}$, then
\[\E{\norm{x^k-x(\lambda)}^2} \leq \left(1- \frac{\alpha \mu}{n}\right)^k \norm{x^0-x(\lambda)}^2 + \frac{2n\alpha \sigma^2}{\mu}.\]
If we choose $\alpha = \frac{1}{2\cL}$, then 
$\frac{\alpha \mu}{n} =  \frac{\mu}{2 \max\left\{\frac{L}{1-p}, \frac{\lambda }{p}\right\} }$
and
\[\frac{2n\alpha \sigma^2}{\mu} = \frac{ \sum\limits_{i=1}^n \left( \frac{1}{1-p} \| \nabla f_i(x_i(\lambda))\|^2 +  \frac{\lambda^2}{p} \|x_i(\lambda) - \overline{x}(\lambda) \|^2 \right)}{ \max\left\{\frac{L}{1-p}, \frac{\lambda }{p}\right\} \mu}.\]
\end{theorem}

\begin{remark}[Full averaging  not supported]
Is a setup such that conditions of Theorem~\ref{thm:local_local_gd} are satisfied and the aggregation update~\eqref{eq:local_buiufg98fb} is identical to full averaging? This is equivalent requiring $0<p<1$ such that $\alpha \lambda =np$. However, we have $\alpha \lambda   \leq \frac{\lambda  }{2\cL}  \leq np$, which means that full averaging is not supported by our theory.
\end{remark}



\subsection{Optimizing the rate and communication} \label{sec:local_rate}

Let us find the parameters $p$ and $\alpha$ which lead to the fastest rate, in terms of either iterations or communication rounds, to push the error within $\varepsilon$ of the neighborhood\footnote{In Section~\ref{sec:local_lsgd} we propose a variance reduced algorithm which is able to get rid of the neighborhood in the convergence result completely. In that setting, our goal will be to achieve $\E{\norm{x^k-x(\lambda)}^2} \leq \varepsilon \norm{x^0-x(\lambda)}^2$.  } from Theorem~\ref{thm:local_local_gd}, i.e., to achieve
\begin{equation}\label{eq:local_bi7g97ibudd} \E{\norm{x^k-x(\lambda)}^2} \leq \varepsilon \norm{x^0-x(\lambda)}^2 + \frac{2n\alpha \sigma^2}{\mu}. \end{equation}



\begin{corollary}\label{cor:local_optimalp}
The value $p^{*} = \frac{\lambda}{L + \lambda}$ minimizes both the number of iterations and the expected number of communications for achieving \eqref{eq:local_bi7g97ibudd}. In particular, the optimal number of iterations is $2\frac{L+\lambda}{\mu} \log \frac{1}{\varepsilon}$, and the optimal expected number of communications is $\frac{2\lambda}{\lambda+ L} \frac{L}{\mu} \log \frac{1}{\varepsilon}$.
\end{corollary}
 

If we choose $p=p^*$, then $\frac{\alpha \lambda }{np} = \frac{1}{2}$, and the aggregation  rule~\eqref{eq:local_buiufg98fb} in Algorithm~\ref{alg:local_L2GD} becomes
\begin{equation}\label{eq:local_bui87g9f}
x^{k+1}_i = \frac12 \left( x^k_i +\bar{x}^k\right) 
\end{equation}
while the local {\tt GD} step~\eqref{eq:local_damkpdaosdaon} becomes
$
x^{k+1}_i  =x^k_i - \frac{1}{2L} \nabla f_i(x_i^k).
$
Notice that while our method does not support full averaging as that is too unstable,  \eqref{eq:local_bui87g9f} suggests that one should take a large step {\em towards} averaging.  

\begin{figure}[t]
\centering
\begin{minipage}{0.5\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{evolution.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\vskip -0.3cm
\caption{Distance of solution $x(\lambda)$ of~\eqref{eq:local_main} to pure local solution $x(0) $ and global solution $x(\infty)$ as a function of $\lambda$. Logistic regression on a1a dataset. See Appendix for experimental setup.} 
\label{fig:local_lambda}
\end{figure}

As $\lambda $ get smaller, the solution to the optimization problem \eqref{eq:local_main} will increasingly favour pure local models, i.e., $x_i(\lambda) \to x_i(0) \eqdef \arg\min f_i$ for all $i$ as $\lambda \to 0$. Pure local models can be computed without any communication whatsoever and Corollary~\ref{cor:local_optimalp} confirms this intuition: the optimal number of communication round decreases to zero as $\lambda \to 0$. On the other hand, as $\lambda \to \infty$, the optimal number of communication rounds converges to $2\frac{L}{\mu}\log \frac{1}{\varepsilon}$, which recovers the performance of {\tt GD} for finding the globally optimal model (see Figure~\ref{fig:local_lambda}). 




{\em In summary, we recover the communication efficiency of {\tt GD} for finding the globally optimal model as $\lambda \to \infty$. However, for other values of $\lambda$, the communication complexity of {\tt L2GD} is better and decreases to $0$ as $\lambda \to 0$. Hence, our communication complexity result interpolates between the communication complexity of {\tt GD} for finding the global model and the zero communication complexity for finding the pure local models. }



\section{The {\tt L2SGD+} algorithm} \label{sec:local_lsgd}


As we have seen in Section~\ref{sec:local_analysis}, {\tt L2GD} is a specific instance of {\tt SGD}, thus only converges linearly to the neighborhood of the optimum. In this section, we resolve the mentioned issue by incorporating control variates to the stochastic gradient~\cite{svrg, saga}.

We also go further. We assume that each local objective has a finite-sum structure and propose an algorithm---{\tt L2SGD+}---which takes \emph{local stochastic} gradient steps, while maintaining (global) linear convergence rate. As a consequence, {\tt L2SGD+} is the first local {\tt SGD} with linear convergence.\footnote{We are aware that a linearly converging local {\tt SGD} (with $\lambda = \infty$) might be obtained as a particular instance of the decoupling method from~\cite{mishchenko2019stochastic}, although this was not stated in the mentioned paper. Other variance reduced local {\tt SGD} algorithms~\cite{liang2019variance, karimireddy2019scaffold, wu2019federated} are not capable of achieving linear convergence.} For the reader's convenience, we present a variance reduced local gradient descent (i.e., no subsampling) in the Appendix. 

\subsection{Setup}
Consider $f_\tRloc(x_{\tRloc}) = \frac1m \sum_{j =1}^m \flocc_{i,j}(x_{\tRloc})$. Therefore, the objective function~\eqref{eq:local_main} becomes
\[
  F(x)  =\frac1n \sum \limits_{\tRloc=1}^{\TRloc} \underbrace{  \left( \frac1m\sum_{j=1}^m\flocc_{i,j}(x_{\tRloc})\right)}_{=  f_{\tRloc}(x) } + \lambda\underbrace{\frac{1}{2\TRloc} \sum_{\tRloc=1}^{\TRloc} \| x_{\tRloc} - \bar{x}\|^2.}_{= \Phi(x)}
\]

\begin{assumption}\label{as:local_smooth_sc_simple}
Function $\flocc_{i,j}$ is convex, $\Lloc$ smooth while $f_i$ is $\mu$-strongly convex (for each $1\leq j \leq m, 1\leq \tRloc \leq \TRloc$).
\end{assumption}
Denote $\onesmloc\in \R^m$ to be vector of ones. We are now ready to state {\tt L2SGD+} as Algorithm~\ref{alg:local_L2SGD}. 


  
  
\begin{algorithm}[h]
  \caption{{\tt L2SGD+}: Loopless Local  {\tt SGD} with Variance Reduction}
  \label{alg:local_L2SGD}
\begin{algorithmic}
\State{\bfseries Input: }{$x^0_1 = \dots = x_{n}^0\in\R^{d}$, stepsize $\alpha$, probability $p$ }
\State $\mJf^0_{\tRloc}  = 0 \in \R^{d\times m}, \mJpsi^0_{\tRloc}  = 0 \in \R^{d}$ (for $\tRloc = 1,\dots, \TRloc$)
  \For{$k=0,1,2,\dotsc$}
  \State $\xi = 1$ with probability $p$ and $0$ with probability $1-p$ 
  \If {$\xi=0$}
 \State All {\color{red}Devices} $i=1,\dots,n$:      
          \State \hskip .3cm Sample $j \in \{1,\dots, m\}$ (uniformly at random)
       \State \hskip .3cm $g^k_\tRloc = \frac{1}{\TRloc(1-\pagg)} \left(\nabla \flocc_{i,j}(x^k_{\tRloc})- \left(\mJf^k_{\tRloc}\right)_{:,j}\right) + \frac{ \mJf^k_{\tRloc} \onesmloc}{\TRloc m}  +   \frac{\mJpsi^k_{\tRloc}}{\TRloc}  $ 
         \State \hskip .3cm $x^{k+1}_\tRloc = x^{k}_\tRloc - \alpha g^k_\tRloc$
        \State  \hskip .3cm Set $(\mJ^{k+1}_i)_{:,j} = \nabla \flocc_{i,j}(x^k_\tRloc)$, $\mJpsi^{k+1}_{\tRloc}= \mJpsi^k_{\tRloc}$,
        \State \hskip 0.83cm  $(\mJ^{k+1}_i)_{:,l} = (\mJ^{k+1}_i)_{:,l} $ for all $l\neq j$
         		\vspace*{-0.1cm}
 \Else 
  \State {\color{blue}Master} computes the average $\bar{x}^k = \frac{1}{n}\sum_{i=1}^n x_i^k$
\State {\color{blue}Master} does for all $i=1,\dots,n$:       
   \State \hskip .3cm $g^k_\tRloc=   \frac{\lambda }{\TRloc \pagg} (x^k_{\tRloc} - \bar{x}^k) - \frac{\pagg^{-1} -1}{ \TRloc}\mJpsi^k_{\tRloc} + \frac{1}{\TRloc m} \mJf_{\tRloc}^k \onesmloc$
 		\State  \hskip .3cm Set $x_{\tRloc}^{k+1} = x_{\tRloc}^k  - \alpha g^k_\tRloc $
 		\State  \hskip .3cm Set $\mJpsi^{k+1}_{\tRloc} =  \lambda (x_{\tRloc}^k - \bar{x}^k )$, $\mJf^{k+1}_{\tRloc} = \mJf^{k}_{\tRloc} $
    \EndIf
      \EndFor
\end{algorithmic}
\end{algorithm}


\begin{remark}
{\tt L2SGD+} is the simplest local {\tt SGD} method with variance reduction. In the Appendix, we present general {\tt L2SGD++} which allows for 1) an arbitrary number of data points per client and arbitrary local subsampling strategy, 2) partial participation of clients, and 3) local {\tt SVRG}-like updates of control variates (thus potentially better memory). Lastly, {\tt L2SGD++} is able exploit the smoothness structure of the local objectives, resulting in tighter rates.
\end{remark}


{\tt L2SGD+} only communicates when a two consecutive coin tosses land a different value, thus, on average $p(1-p)k$ times per $k$ iterations. However, {\tt L2SGD+} requires communication of control variates $\mJf_i \onesmloc,  \mJpsi_i$ as well -- each communication round is thus three times more expensive. In the Appendix, we provide an implementation of {\tt L2SGD+} that does not require the communication of $\mJf_i \onesmloc,  \mJpsi_i$.

\subsection{Theory}

%
We are now ready to present a convergence rate of {\tt L2SGD+}.



\begin{theorem} \label{thm:local_saga_simple}

Let Assumption~\ref{as:local_smooth_sc_simple} hold and choose
$  \alpha =\TRloc \min \left \{  \frac{(1-\pagg) }{ 4  \Lloc + \mu m} , \frac{\pagg}{4\lambda+ \mu} \right\}.$
Then the iteration complexity of Algorithm~\ref{alg:local_L2SGD} is 
$  \max \left\{   \frac{4\Lloc  + \mu m}{ (1-\pagg)\mu}, \frac{4\lambda +\mu}{\pagg\mu}\right \}\log\frac1\varepsilon.$
\end{theorem}

Next, we find a probability $p$ that yields both the best iteration and communication complexity. 

\begin{corollary}\label{cor:local_lsd_optimal_p}
Both communication and iteration complexity of {\tt L2SGD+} are minimized for $\pagg  = \frac{4\lambda +\mu}{4\lambda +4\Lloc +(m+1)\mu}$. The resulting iteration complexity is $\left(4 \frac{\lambda }{\mu} +4 \frac{\Lloc}{\mu} +m+1\right) \log \frac1\varepsilon$, while the communication complexity is $\frac{4 \lambda + \mu }{4\Lloc + 4 \lambda + (m+1)\mu} \left( 4\frac{\Lloc}{\mu}+m\right) \log \frac{1}{\varepsilon}$. 
\end{corollary}

Note that with $\lambda \rightarrow \infty$, the communication complexity of {\tt L2SGD+} tends to $ \left( 4\frac{\Lloc}{\mu}+m\right) \log \frac{1}{\varepsilon}$, which is communication complexity of minibatch {\tt SAGA} to find the globally optimal model (see Chapter~\ref{jacsketch}). On the other hand, in the pure local setting ($\lambda=0$), the communication complexity becomes $\log \frac1\epsilon$ -- this is because the Lyapunov function involves a term that measures the distance of local models, which requires communication to be estimated.

\begin{figure}[th]
\centering
\begin{minipage}{0.5\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{commp2loglog.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\caption{ Communication rounds to get $\frac{F(x^k)-F(x^*)}{F(x^0)-F(x^*)}\leq 10^{-5}$ as a function of $p$ with $p^* \approx 0.09$ (for {\tt L2SGD+}). Logistic regression on a1a dataset with $\lambda = 0.1$; details in the Appendix. } 
\label{fig:local_comm_p}
\end{figure}




\section{Experiments \label{sec:local_exp}}
In this section, we numerically verify the theoretical claims from this chapter.  In all experiments in this chapter, we consider a simple binary classification model -- logistic regression. In particular, suppose that device $i$ owns data matrix $\mA_{i}\in \R^{m \times d}$ along with corresponding labels $b_{i}\in \{-1, 1\}^{m}$. The local objective for client $i$ is then given as follows
\[
f_{i}(x) \eqdef  \frac1m \sum_{j=1}^m \flocc_{i, j}(x) +\frac{\mu}{2} \| x\|^2, \quad \text{where} \quad \flocc_{i m+ j}(x) \eqdef \log \left(1+\exp\left((\mA_{i})_{j,:}x\cdot  b_{i}\right) \right).
\]
The rows of data matrix $\mA$ were normalized to have length 4 so that each $\flocc_{i,j}$ is $1$-smooth for each $j$. At the same time, the local objective on each device is $10^{-4}$-strongly convex. Next, datasets are from LibSVM~\cite{chang2011libsvm}. 

In each case, we consider the simplest locally stochastic algorithm. In particular, each dataset is evenly split among the clients, while the local stochastic method samples a single data point each iteration. 


We have chosen a different number of clients for each dataset -- so that we cover different possible scenarios. See Table~\ref{tbl:local_data} for details (it also includes sizes of the datasets). Lastly, the stepsize was always chosen according to Theorem~\ref{thm:local_saga_simple}.



\begin{table}[!h]
\caption{Setup for the experiments.}
\label{tbl:local_data}
\begin{center}
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Dataset &  \begin{tabular}{c} $\nlocc$ \\ $=\TRloc m$ \end{tabular}   & $d$ &  $\TRloc$ & $m$   & $\mu$&$L$& \begin{tabular}{c} $\pagg$ \\ \ref{sec:local_exp_comp} \end{tabular} & \begin{tabular}{c} $\lambda$ \\ \ref{sec:local_exp:pagg} \end{tabular} & \begin{tabular}{c} $\pagg$ \\ \ref{sec:local_exp:omega} \end{tabular}\\
\hline
\hline
\texttt{a1a} & 1 605	& 123 & 5 & 321 & $10^{-4}$ & $1$&0.1 &0.1 &0.1\\ \hline
\texttt{mushrooms} & 8 124 & 112 & 12 &677 & $10^{-4}$ & $1$ &0.1 & 0.05 & 0.3 \\ \hline
\texttt{phishing} & 11 055	&	68 & 11 & 1 005 & $10^{-4}$ & $1$ &0.1 &0.1 & 0.001\\ \hline
\texttt{madelon} & 2 000& 500& 50 &40 & $10^{-4}$& $1$ &0.1  &0.02&0.05\\ \hline
\texttt{duke} &44 & 7 129& 4 & 11& $10^{-4}$ & $1$ & 0.1 & 0.4&0.1\\ \hline
\texttt{gisette\_scale} & 6 000& 5 000& 100 & 60 & $10^{-4}$ & $1$&0.1 &0.2&0.003  \\ \hline
\texttt{a8a} &22 696 & 123& 8 & 109& $10^{-4}$ & $1$ &0.1&0.1  &0.1\\ \hline
\end{tabular}
%\end{adjustbox}
\end{center}
\end{table}











\subsection{Comparison of the methods \label{sec:local_exp_comp}}


In our first experiment, we verify two phenomena:
\begin{itemize}
\item Effect of variance reduction on the convergence speed of local methods. We compare 3 different methods: local {\tt SGD} with full variance reduction (Algorithm~\ref{alg:local_L2SGD}), shifted local {\tt SGD} (Algorithm~\ref{alg:local_lsgd_partial}) and local {\tt SGD} (Algorithm~\ref{alg:local_lsgd_none}). Our theory predicts that a fully variance reduced algorithm converges to the global optimum linearly, while both shifted local {\tt SGD} and local {\tt SGD} converge to a neighborhood of the optimum. At the same time, the neighborhood should be smaller for shifted local {\tt SGD}. 


\item The claim that heterogeneity of the data does not influence the convergence rate. We consider two splits of the data heterogeneous and homogenous. For the homogenous split, we first randomly reshuffle the data and then construct the local objectives according to the current order (i.e., the first client owns the first $m$ indices, etc.). For heterogenous split, we first sort the data based on the labels and then construct the local objectives accordingly (thus achieving the worst-case heterogeneity). Note that the overall objective to solve is different in homogenous and heterogenous case -- we thus plot relative suboptimality of the objective (i.e., $\frac{F(x^k)-F(x^{*})}{F(x^0)-F(x^{*})}$) to directly compare the convergence speed. 
\end{itemize} 

In all cases, we choose $\pagg=0.1$ and $\lambda = \frac19$ -- such choice mean that $\pagg$ is very close to optimal. The other parameters (i.e. number of clients) are provided in Table~\ref{tbl:local_data}. Figure~\ref{fig:local_libsvm_methods} presents the result.

\begin{figure}[!h]
\centering
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{method_exp_epochDataseta1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{method_exp_epochDatasetmushrooms.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{method_exp_epochDatasetphishing.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{method_exp_epochDatasetmadelon.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{method_exp_epochDatasetduke.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{method_exp_epochDatasetgisette_scale.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{method_exp_epochDataseta8a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\caption{Variance reduced local {\tt SGD} (Algorithm~\ref{alg:local_L2SGD}), shifted local {\tt SGD} (Algorithm~\ref{alg:local_lsgd_partial}) and local {\tt SGD} (Algorothm~\ref{alg:local_lsgd_none}) applied on LibSVM problems for both homogenous split of data and Heterogenous split of the data. Stepsize for non-variance reduced method was chosen the same as for the analogous variance reduced method.} 
\label{fig:local_libsvm_methods}
\end{figure}


As expected, Figure~\ref{fig:local_libsvm_methods} clearly demonstrates the following: 
\begin{itemize}
\item Full variance reduction always converges to the global optima, methods with partial variance reduction only converge to a neighborhood of the optimum.
\item Partial variance reduction (i.e., shifting the local {\tt SGD}) is better than not using control variates at all. Although the improvement in the performance is rather negligible.
\item Data heterogeneity does not affect the convergence speed of the proposed methods. Therefore, unlike standard local {\tt SGD}, mixing the local and global models does not suffer the problems with heterogeneity.
\end{itemize}

\subsection{Effect of $\pagg$\label{sec:local_exp:pagg}}

In the second experiment, we study the effect of $\pagg$ on the convergence rate of variance reduced local {\tt SGD}. Note that $\pagg$ immediately influences the number of communication rounds -- on average, the clients take $(\pagg^{-1}-1)$ local steps in between two consecutive rounds of communication (aggregation). 

In Section~\ref{sec:local_lsgd}, we argue that, it is optimal (in terms of the convergence rate) to choose $\pagg$ of order $\pagg^{*}\eqdef \frac{\lambda}{\Lloc+\lambda}$. Figure~\ref{fig:local_libsvm_pagg} compares $\pagg=  \pagg^{*}$ against other values of $\pagg$ and confirms its optimality (in terms of optimizing the convergence rate). 

While the slower convergence of Algorithm~\ref{alg:local_L2SGD} with $\pagg<\pagg^{*}$ is expected (i.e., communicating more frequently yields a faster convergence), slower convergence for $\pagg>\pagg^{*}$ is rather surprising; in fact, it means that communicating less frequently yields faster convergence. This effect takes place due to the specific structure of problem~\eqref{eq:local_main}; it would be lost when enforcing $x_1=\dots = x_{\TRloc}$ (corresponding to $\lambda=\infty$).



\begin{figure}[!h]
\centering
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{pagg_exp_epochDataseta1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{pagg_exp_epochDatasetmushrooms.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{pagg_exp_epochDatasetphishing.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{pagg_exp_epochDatasetmadelon.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{pagg_exp_epochDatasetduke.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{pagg_exp_epochDatasetgisette_scale.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{pagg_exp_epochDataseta8a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\caption{Effect of the aggregation probability $\pagg$ (legend of the plots) on the convergence rate of Algorithm~\ref{alg:local_L2SGD}. Choice $\pagg = \pagg^{*}$ corresponds to red dotted line with triangle marker. Parameter $\lambda$ was chosen in each case as Table~\ref{tbl:local_data} indicates. } 
\label{fig:local_libsvm_pagg}
\end{figure}


\subsection{Effect of $\lambda$ \label{sec:local_exp:omega}}
In this experiment we study how different values of $\lambda$ influence the convergence rate of Algorithm~\ref{alg:local_L2SGD}, given that everything else (i.e. $\pagg$) is fixed. Note that for each value of $\lambda$ we get a different instance of problem~\eqref{eq:local_main}; thus the optimal solution is different as well. Therefore, in order to make a fair comparison between convergence speeds, we plot the relative suboptimality (i.e. $\frac{F(x^k)-F(x^{*})}{F(x^0)-F(x^{*})}$) against the data passes. Figure~\ref{fig:local_libsvm_omega} presents the results.


The complexity of Algorithm~\ref{alg:local_L2SGD} is\footnote{Given that $\mu$ is small.} $\cO\left(\frac{\Lloc}{(1-\pagg)\mu} \right)\log\frac1\varepsilon$ as soon as $\lambda< \lambda^{*} \eqdef \frac{L\pagg}{(1-\pagg)}$; otherwise the complexity is $\cO\left(\frac{\lambda}{\pagg\mu} \right)\log\frac1\varepsilon$. This perfectly consistent with what  Figure~\ref{fig:local_libsvm_omega} shows -- the choice $\lambda<\lambda^{*}$ resulted in comparable convergence speed than $\lambda=\lambda^{*}$; while the choice $\lambda>\lambda^{*}$ yields noticeably worse rate than $\lambda=\lambda^{*}$.







\begin{figure}[!h]
\centering
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{omega_exp_epochDataseta1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{omega_exp_epochDatasetmushrooms.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{omega_exp_epochDatasetphishing.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{omega_exp_epochDatasetmadelon.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{omega_exp_epochDatasetduke.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{omega_exp_epochDatasetgisette_scale.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{omega_exp_epochDataseta8a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:local_bl_ex_flops}
\end{minipage}%
\caption{Effect of parameter $\lambda$ (legend of the plot) on the convergence rate of Algorithm~\ref{alg:local_L2SGD}. The choice $\lambda=\lambda^{*}$ corresponds to borwn dash-dotted line with diamond marker (the third one from the legend). Aggregation probability $\pagg$ was chosen in each case as Table~\ref{tbl:local_data} indicates. } 
\label{fig:local_libsvm_omega}
\end{figure}






\section{Conclusion}

In this chapter we have proposed a new optimization formulation for federated learning. The algorithms (i.e., {\tt L2GD}) we propose to solve the new formulation are similar the classical local {\tt SGD}, however, the rates we have provided are superior to classical local {\tt SGD} analysis. 

Our analysis of {\tt L2GD} can be extended to cover smooth convex and non-convex loss functions $f_i$ (we do not explore these directions). Further, our methods can be extended to a decentralized regime where the devices correspond to devices of a connected network, and communication is allowed along the edges of the graph only. This can be achieved by introducing an additional randomization over the penalty $\Phi$. Further, our approach can be accelerated in the sense of Nesterov~\cite{nesterov2018lectures} by adapting the results from \cite{allen2017katyusha, l-svrg-as} to our setting, thus further reducing the number of communication rounds.

==> sscn.tex <==
\chapter{Stochastic Subspace Cubic Newton Method}
\label{sscn}



\graphicspath{{sscn/plots/}}



In this chapter we consider a regularized not necessarily finite-sum optimization problem 
\begin{equation}\label{eq:sscn_problem}
    \min_{x \in \R^d}  \, \left \{ F(x) \eqdef f(x) + \psi(x)\right \},
\end{equation}
where $f:\R^d\to \R$ is convex and twice differentiable and $\psi:\R^d\to \R\cup \{+\infty\}$ is a proximable convex function. We are interested in the regime where the dimension $d$ is very large, which arises in many contexts, such as  the training of modern over-parameterized machine learning models. In this regime, coordinate descent ({\tt CD}) methods, or more generally subspace descent methods, are the methods of choice. 

\section{Subspace descent methods}

Subspace descent methods rely on  update rules of the form
\begin{equation} \label{eq:sscn_update_general}
x^+ = x + \mS h,\qquad \mS \in \R^{d\times \tau(\mS)}, \qquad h\in \R^{\tau(\mS)},
\end{equation}
where $\mS$ is a thin matrix, typically with a negligible number of columns compared to the dimension (i.e., $\tau(\mS)\ll d$). That is, they move from $x$ to $x^+$ along the subspace spanned by the columns of $\mS$.

In these methods,  the subspace matrix $\mS$ is typically chosen first, followed by the determination of the parameters $h$ which define the linear combination of the columns determining the update direction. Several different rules have been proposed in the literature for choosing the matrix $\mS$, including greedy,  cyclic and randomized rules. In this work we consider a \textit{randomized} rule. In particular, we assume that $\mS$ is sampled from an arbitrary but fixed distribution $\cD$ restricted to requiring that $\mS$ be of full column rank\footnote{It is rather simple to extend our results to matrices $\mS$ which are column-rank deficient. However, this would introduce a rather heavy notation burden which we decided to avoid for the sake of clarity and readability.} with probability one. 

Once $\mS\sim \cD$ is sampled, a rule for deciding  the stepsize $h$ varies from algorithm to algorithm, but is mostly determined by the underlying \emph{oracle model} for information access to function $f$. For instance, first-order methods require  access to the subspace gradient $\nabla_{\mS} f(x) \eqdef  \mS^\top \nabla f(x)$, and are relatively well studied~\cite{rcdm, stich2013optimization, richtarik2014iteration, wright2015coordinate, kozak2019stochastic}. At the other extreme are  variants performing a full subspace minimization, i.e.,  $f$ is minimized over the affine subspace given by $\{ x+\mS h \, | \, h\in \R^{\tau(\mS)}\}$~\cite{chang2008coordinate}.  In particular, in this chapter we are interested in the \emph{second-order} oracle model; i.e. we claim access both to the subspace gradient $\nabla_{\mS} f(x)$ and the subspace Hessian $\nabla^2_{\mS} f(x)\eqdef \mS^\top \nabla^2f(x)\mS$.

\section{Contributions}

We now summarize our contributions:

\begin{itemize}
\item {\bf New 2nd order subspace method.} We propose a new stochastic subspace method---Stochastic Subspace Cubic Newton ({\tt SSCN})---constructed by minimizing an oracle-consistent global upper bound on the objective $f$ in each iteration (Section~\ref{sec:sscn_Alg}). This bound is formed using both the subspace gradient and the subspace Hessian at the current iterate and relies on Lipschitzness of the subspace Hessian. 

\item {\bf Interpolating global rate.} We prove (Section~\ref{sec:sscn_global}) that {\tt SSCN} enjoys a global convergence rate that interpolates between the rate of stochastic {\tt CD} and the rate of cubic regularized Newton as one varies the expected dimension of the subspace, $\E{\tau(\mS)}$. 

\item {\bf Fast local rate.} Remarkably, we establish a local convergence bound for {\tt SSCN}  (Section~\ref{sec:sscn_local}) that matches the rate of stochastic subspace descent ({\tt SSD})~\cite{gower2015randomized} applied to solving the problem \begin{equation} \label{eq:sscn_quadratic_optimum}
 \min_{x \in \R^d}\; \frac12 (x-x^*)^\top \nabla^2f(x^*)(x-x^*),
\end{equation} where $x^*$ is the solution of~\eqref{eq:sscn_problem}. Thus, {\tt SSCN} behaves as {\em if} it had access to a perfect second-order model of $f$ at the optimum, and was given the (intuitively much simpler) task of minimizing this model instead. 
Furthermore, note that {\tt SSD}~\cite{gower2015randomized} applied to minimize a convex quadratic can be interpreted as doing an exact subspace search in each iteration, i.e., it minimizes the objective exactly along the active subspace~\cite{richtarik2017stochastic}. Therefore, the local rate of {\tt SSCN} matches the rate of the greediest strategy for choosing $h$ in the active subspace, and as such, this rate is the best one can hope for a method that does not incorporate some form of acceleration.

\item {\bf Special cases.} We discuss in Section~\ref{sec:sscn_special} how {\tt SSCN} reduces to several existing stochastic second-order methods in special cases, either recovering the best known rates, or improving upon them. This includes  {\tt  SDSA}~\cite{sda}, {\tt CN}~\cite{griewank1981modification, nesterov2006cubic} and {\tt RBCN}~\cite{doikov2018randomized}. However, our method is more general and hence allows for more applications.

\end{itemize}

We discuss more remotely related literature in Section~\ref{sec:sscn_related_literature}. We now give a simple example of our setting.

\begin{example}[Coordinate subspace setup]
Let $\mI^d\in \R^{d\times d}$ be the identity and let $S$ be a random subset of $\{1, 2, \dots, d \}$. Given that $\mS = \mI^d_{(:,S)}$ with probability 1, the oracle model reveals $(\nabla f(x))_S$ and $(\nabla^2 f(x))_{(S,S)}$. Therefore, we have access to a random block of partial derivatives of $f$ and a block submatrix of its Hessian, both corresponding to the subset of indices $S$. Furthermore, the rule~\eqref{eq:sscn_update_general} updates a subset $S$ of coordinates only. In this setting, our method is a new \textit{second-order coordinate subspace descent} method.
\end{example}


\section{Preliminaries \label{sec:sscn_preliminaries}}

Throughout the chapter, we assume that  $f$ is convex, twice differentiable, and sufficiently smooth and that $\psi$ is convex, albeit possibly non-differentiable, as the next assumption states.\footnote{We will also require separability of $\psi$; see Section~\ref{sec:sscn_setup}.}

\begin{assumption}\label{as:sscn_conv_lipschitz}
Function $f: \R^d \to \R$ is convex and twice differentiable with $M$-Lipschitz continuous Hessian. Function $\psi: \R^d \to \R \cup \{ +\infty \}$ is  proper closed and convex.
\end{assumption}

We always assume that a minimum of $F$  exists and by  $x^*$ denote any of its minimizers. We let $F^{*} \eqdef F(x^{*})$. 


Since our method always takes steps along random subspaces spanned by the columns of $\mS \in \R^{d\times \tau(\mS)}$,  it is reasonable to define the Lipschitzness of the Hessian over the range of $\mS$:\footnote{By  $\|x\| \eqdef \la x, x \ra^{1/2}$we denote the standard Euclidean norm.}
\begin{equation}\label{eq:sscn_MS_def}
M_{\mS}  \eqdef \max_{x\in \R^d} \max_{\substack{  \;\; h \in \R^{\tau(\mS)}, \\ h \not= 0 } } \frac{ |\nabla^3 f(x)[\mS h]^3| }{\|\mS h\|^3}\, .
\end{equation}

As the next lemma shows,  the maximal value of $M_{\mS}$ for any $\mS$ of width $\tau$ can be up to $(\frac{d}{\tau})^{\frac32}$ times smaller than $M$ and this will lead to  a tighter approximation of the objective. 
\begin{lemma} \label{lem:sscn_sharpness}
We have $
M \geq \max_{\tau(\mS) = \tau }M_{\mS}.
$
Moreover, there is a problem where $ \max_{\tau(\mS) = \tau}M_{\mS} =\left(\frac{\tau}{d}\right)^{\frac32} M$. Lastly, if $\Range{\mS} = \Range{\mS'}$, then  $M_{\mS} = M_{\mS'}$.
\end{lemma}


The next lemma provides a direct motivation for our algorithm. It gives a global upper bound on the objective over a random subspace, given the first and second-order information at the current point. 

\begin{lemma}\label{lem:sscn_ub}
Let $x\in \R^d$, $\mS\in \R^{d\times \tau(\mS)}$, $h\in \R^{\tau(\mS)}$ and $x^+$ be as in \eqref{eq:sscn_update_general}. Then
\begin{equation}
\left | f(x^+) -  f(x)  - \langle \nabla_{\mS} f(x), h \rangle - \frac12 \la \nabla^2_{\mS}f(x) h, h\ra \right |   \leq  \frac{M_{\mS}}{6} \| \mS h\|^3. \label{eq:sscn_coordinate_ub}
\end{equation}
As a consequence, we have
\begin{eqnarray} 
F(x^+) \leq  F(x) + T_{\mS}(x,h),
\label{eq:sscn_coordinate_ub_full}
\end{eqnarray}
where
$T_{\mS}(x,h) \eqdef \langle \nabla_{\mS} f(x), h \rangle + \frac12 \la  \nabla^2_{\mS}  f(x) h, h \ra
+  \frac{M_{\mS}}{6} \| \mS h\|^3 + \psi(x+\mS h).$
\end{lemma}

We shall also note that for function $\psi$
we require \textit{separability} with respect to the sampling distribution
(see Definition~\ref{def:separable} and the corresponding
Assumption~\ref{as:sscn_separable} in Section~\ref{sec:sscn_setup}).

For better orientation throughout the chapter, we provide a table of frequently used notation in the Appendix.


\section{The {\tt SSCN} algorithm} \label{sec:sscn_Alg}




For a given $\mS$ and current iterate $x^k$, it is a natural idea to choose $h$ as a minimizer of the upper bound~\eqref{eq:sscn_coordinate_ub_full} in $h$ for $x=x^k$, and subsequently set $x^{k+1} = x^+$ via~\eqref{eq:sscn_update_general}.  Note that we are choosing $\mS$ randomly according to a fixed distribution $\cD$ (with a possibly random number of columns). We have just described {\tt SSCN}---Stochastic Subspace Cubic Newton---formally stated as  Algorithm~\ref{alg:sscn_crcd}.
 
\begin{algorithm}[!h]
\begin{algorithmic}[1]
\State \textbf{Initialization:} $x^0$, distribution $\cD$ of random matrices with $d$ rows and full column rank
\For{$k =  0, 1, 2,\dots$}
\State Sample $\mS$ from distribution $\cD$
\State $h^k =  \argmin_{h \in \R^{\tau(\mS)}}  T_{\mS}(x^k,h)$
\State Set $x^{k+1}=x^k + \mS h^k$ \label{eq:sscn_x_update_CRCD}
\EndFor
\end{algorithmic}
\caption{{\tt SSCN}: Stochastic Subspace Cubic Newton}
\label{alg:sscn_crcd}
\end{algorithm}

\begin{remark}\label{rem:monotonic}
Inequality~\eqref{eq:sscn_coordinate_ub_full} becomes an equality with $h=0$. As a consequence, we must have $F(x^{k+1}) \leq F(x^k)$, and thus the sequence $\{ F(x^k) \}_{k \geq 0}$ is non-increasing.
\end{remark}

\subsection{Solving the subproblem \label{sec:sscn_solving}}
Algorithm~\ref{alg:sscn_crcd} requires $T_{\mS}$ to be minimized in $h$ each iteration. As this operation does not have a closed-form solution in general, it requires an optimization subroutine itself of a possibly non-trivial complexity, which we discuss here. 

\paragraph{The subproblem without $\psi$.}
Let us now consider the case when  $\psi(x) \equiv 0$ in which our problem~\eqref{eq:sscn_problem} does not contain any nondifferentiable components. Various techniques for minimizing regularized quadratic functions were developed  during the development of
Trust-region methods (see~\cite{conn2000trust}), and applied
to Cubic regularization in~\cite{nesterov2006cubic}. The classical approach consists in performing some diagonalization of the matrix $\nabla^2_{\mS} f(x)$ first, by computing the \textit{eigenvalue} or \textit{tridiagonal} decomposition, which costs $\cO(\tau(\mS)^3)$ arithmetical operations.
Then, to find the minimizer, it merely remains to solve a one-dimensional nonlinear equation (this part can be done by $\tilde{\cO}(1)$ iterations of the one-dimensional Newton method, with a linear cost per step). More details and analysis of this procedure can be found
in~\cite{gould2010solving}.


The next example gives a setting in which  an explicit formula for the minimizer of $T_{\mS}$ can be deduced.
\begin{example}\label{ex:explicit} 
Let $e_i$ be the $i$th unit basis vector in $\R^d$. If $\mS\in \{e_1, \dots, e_d\}$ with probability 1 and $\psi(x) = 0$, the update rule can be written as
$x^{k+1} = x^k - \alpha_i^k e_i,$ with
\[
\alpha_i^k = \frac{2\nabla_i f(x^{k})}{\nabla^2_i f(x^{k}) + \sqrt{\left(\nabla^2_{ii} f(x^{k})  \right)^2 + 2M_{e_i}|\nabla_i f(x^{k}) |} },
\]
thus the cost of solving the subproblem is $\cO(1)$.
\end{example}

\paragraph{Subproblem with simple $\psi$.} In some scenarios, minimization of $T_{\mS}$  can be done using a simple algorithm if $\psi$ is simple enough. We now give an example of this.
%In the introduction, we mentioned that the regularizer $\psi$ should be ``simple''. By this, we mean that $\psi$ should not be the bottleneck in minimizing $T_{\mS}$.

\begin{example} 
	If $\mS\in \{e_1, \dots, e_d\}$ with probability 1, the subproblem can be solved using a binary search given that the evaluation of $\psi$ is cheap. In particular, if we can evaluate $\psi(x^k+ \mS h)- \psi(x^k)$ in $\tilde{\cO}(1)$, the cost of solving the subproblem will be $\tilde{\cO}(1)$.
\end{example}

\paragraph{The subproblem with general $\psi$.} In the case of general regularizers, recent line of work \cite{carmon2019gradient} explores to the use
of \textit{first-order} optimization methods (Gradient Methods) for
computing an approximate minimizer of $T_{\mS}$.
We note that the backbone of such Gradient Methods is an implementation of the following operation 
(for a any given vector $b \in \R^{\tau(\mS)}$, and positive scalars $\alpha, \beta$):
\[
 \argmin \limits_{h \in \R^{\tau(\mS)}} \la b, h \ra + \frac{\alpha}{2}\|\mS h\|^2 + \frac{\beta}{3}\|\mS h\|^3 + \psi(x^k + \mS h).
\]

To the best of our knowledge, the most efficient gradient method is the Fast Gradient Method ({\tt FGM})\cite{nesterov2019inexact}, achieving an $\cO(1/k^6)$ convergence rate. However, {\tt FGM} can deal with any $\psi$ as long as the above subproblem is cheap to solve. We shall also note that gradient methods do not require a storage of $\nabla^2_{\mS} f(x)$; but rather iteratively access partial Hessian-vector products $\nabla^2_{\mS} f(x) h$.



\paragraph{Line search.}

Note that in Algorithm~\ref{alg:sscn_crcd} we use the Lipschitz constants $M_{\mS}$ 
of the subspace Hessian (see Definition~\eqref{eq:sscn_MS_def}) as the regularization parameters. In many application, $M_{\mS}$ can be estimated cheaply (see Section~\ref{sec:sscn_applications}). In general, however, $M_\mS$ might be unknown or hard to estimate. 
In such a case, one might use a simple one-dimensional search on each iteration: multiply the estimate of $M_\mS$ by the factor of two until the bound~\eqref{eq:sscn_coordinate_ub_full} is satisfied, and divide it by two at the start of each iteration. Note that the average number of such line search steps per iteration can be bounded by two (see~\cite{grapiglia2017regularized} for the details).



\subsection{Special cases} \label{sec:sscn_special}
There are several scenarios where {\tt SSCN} becomes an already known algorithm.  We list them below.

\paragraph{Quadratic minimization.}  If $M=0$ and $\psi = 0$, {\tt SSCN} reduces to the stochastic dual subspace ascent ({\tt SDSA}) method~\cite{sda}, first analyzed in an equivalent primal form as a \emph{sketch-and-project} method in~\cite{gower2015randomized}. In such a case, {\tt SSCN} performs both first-order, second-order updates, and exact minimization over a subspace at the same time due to the quadratic structure of the objective~\cite{richtarik2017stochastic}. The convergence rate we provide in Section~\ref{sec:sscn_local} exactly matches the rate of sketch-and-project as well. As a consequence, we recover a subclass of matrix inversion algorithms~\cite{pseudoinverse} together with stochastic spectral (coordinate) descent~\cite{kovalev2018stochastic} along with their convergence theory. 


\paragraph{Full-space method.} If $\mS=\mI^d$ with probability 1, {\tt SSCN} reduces to cubically regularized Newton ({\tt CN})~\cite{griewank1981modification, nesterov2006cubic}. In this case, we recover both existing global convergence rates and superlinear local convergence rates.  

\paragraph{Separable non-quadratic part of $f$.} The {\tt RBCN} method~\cite{doikov2018randomized} aims to minimize~\eqref{eq:sscn_problem} with $f(x) = g(x) + \phi(x)$, where $g,\phi$ are both convex, and $\phi$ is separable.\footnote{Separability is defined in Section~\ref{sec:sscn_setup}.}
They assume that $\nabla^2 g(x) \preceq \mA \in \R^{d\times d}, \forall x \in \R^d$, while $\phi$ has Lipschitz continuous Hessian. In each iteration, {\tt RBCN} constructs an upper bound on the objective using first-order information from $g$ only. This is unlike {\tt SSCN}, which uses second-order information from $g$. In a special case when $\nabla^2 g(x) = \mA$ for all $x$, {\tt SSCN} and {\tt RBCN} are identical algorithms. However, {\tt RBCN} is less general: it requires separable $\phi$, and thus does not cover some of our applications, and takes directions along coordinates only. Further, the rates we provide are better even in the setting where the two methods coincide ($\nabla^2 g(x)=\mA$). The simplest way to see that is by looking at local convergence -- {\tt RBCN} does not achieve the local convergence rate of block {\tt CD} to minimize~\eqref{eq:sscn_quadratic_optimum}, which is the best one might hope for. 


Besides these particular cases, for a general twice-differentiable $f$, {\tt SSCN} is a new second-order method.
 
\section{Related literature} \label{sec:sscn_related_literature}

Several methods in the literature are related to {\tt SSCN}. We briefly review them below.

\begin{itemize}
\item \emph{Cubic regularization of Newton method} was proposed first in~\cite{griewank1981modification},
and received substantial attention after the work of Nesterov~\cite{nesterov2006cubic}, where its global complexity guarantees were established.
During the last decade, there was a steady increase of research in second-order methods, 
discovering Accelerated~\cite{nesterov2008accelerating,monteiro2013accelerated},
Adaptive~\cite{cartis2011adaptive1,cartis2011adaptive2}, and
Universal~\cite{grapiglia2017regularized,grapiglia2019accelerated,doikov2019minimizing} 
schemes (the latter ones are adjusting automatically  to the smoothness properties of the objective).



\item There is a vast literature on \emph{first-order coordinate descent ({\tt CD})} methods. While {\tt CD} with $\tau=1$ is consistently the same method within the literature~\cite{rcdm, richtarik2014iteration, wright2015coordinate}, there are several ways to deal with $\tau>1$. The first approach constructs a separable upper bound on the objective (in expectation) in the direction of a random subset of coordinates~\cite{qu2016coordinate1, qu2016coordinate2}, which is minimized to obtain the next iterate. The second approach---{\tt SDNA}~\cite{sdna}---works with a tighter non-separable upper bound. {\tt SDNA} is, therefore, more costly to implement but requires a smaller number of iterations to converge. The literature on first-order subspace descent algorithms is slightly less rich, the notable examples are random pursuit~\cite{stich2013optimization} or stochastic subspace descent~\cite{kozak2019stochastic}.




\item \emph{Randomized subspace Newton} ({\tt RSN})~\cite{gower2019rsn} is a method of the form $$x^{k+1} = x^k - \hat{L}^{-1} \mS \left(\nabla^2_\mS f(x^k)\right)^{-1} \nabla_{\mS} f(x^k)$$ for some specific fixed $\hat{L}$. In particular, it can be seen as a method minimizing the following upper bound on the function, which follows from their assumption:
\begin{align*}
 & h^k = \argmin_h\, \langle \nabla_{\mS} f(x^k), h  \rangle + \frac{\hat{L}}{2}  \la \nabla^2_{\mS}  f(x^k) h, h \ra. 
\end{align*}
This is followed by an update over the subspace: $ x^{k+1} = x^k + \mS h^k$. 
Since both {\tt RSN} and {\tt SSCN} are analyzed under different assumptions, the global linear rates are not directly comparable. However, the local rate of {\tt SSCN} is superior to {\tt RSN}. We shall also note that {\tt RSN} is a stochastic subspace version of a method from~\cite{karimireddy2018global}.

\item \emph{Subsampled Newton} (SN) methods~\cite{byrd2011use, erdogdu2015convergence, xu2016sub, roosta2019sub} and \emph{subsampled cubic regularized Newton methods}~\cite{kohler2017sub, xu2017newton, wang2018stochastic} and \emph{stochastic (cubic regularized) Newton methods}~\cite{tripuraneni2018stochastic,cartis2018global, kovalev2019stochastic} are  stochastic second-order algorithms to tackle finite sum minimization. Their major disadvantage is a requirement of an immense sample size, which makes them often impractical if used as theory prescribes. A notable exception that does not require a large sample size was recently proposed in~\cite{kovalev2019stochastic}. However, none of these methods are directly comparable to {\tt SSCN} as they are not subspace descent methods, but rather randomize over data points (or sketch the Hessian from ``inside''~\cite{pilanci2017newton}). 

\end{itemize}


\section{Global complexity bounds}
\label{sec:sscn_global}

We first start presenting the global complexity results of {\tt SSCN}.


\subsection{Setup~\label{sec:sscn_setup}}


Throughout this section, we require some kind of uniformity of the distribution $\cD$ over subspaces given by $\mS$. In particular, we require $\mZ= \mZ(\mS) \eqdef \mS \left(\mS^\top \mS \right)^{-1} \mS^\top$, the projection matrix onto the range of $\mS$, to be a scalar multiple of identity matrix in expectation. 
\begin{assumption}\label{as:sscn_uniform}
$\exists \tau>0$ such that distribution  $\cD$ satisfies
\begin{equation} \label{eq:sscn_uniform_sampling}
\E{\mZ} = \frac{\tau}{d} \mI^d.
\end{equation}
\end{assumption}
A direct consequence of Assumption~\ref{as:sscn_uniform} is that $\tau$ is an expected width of $\mS$, as the next lemma states.
\begin{lemma}\label{lem:sscn_exp_size}
If Assumption~\ref{as:sscn_uniform} holds, then $\E{\tau(\mS)} = \tau$.
\end{lemma}

As mentioned before, the global complexity results are interpolating between convergence rate of (first-order) {\tt CD} and (global) convergence rate of Cubic Newton. However, first-order {\tt CD} requires Lipschitzness of gradients, and thus we will require it as well.
\begin{assumption}\label{as:sscn_smooth}
Function $f$ has $L$-Lipschitz continuous gradients, i.e. $\nabla^2 f(x) \preceq L \mI^d$ for all $x\in \R^d$.
\end{assumption}


We will also need an extra assumption on $\psi$. It is well known that proximal (first-order) {\tt CD} with fixed step size does not converge if $\psi$ is not separable -- in such case, even if $f(x^k) = f(x^*)$ we might have $f(x^{k+1})> f(x^*)$. Therefore, we might not hope that {\tt SSCN} will converge without additional assumptions on $\psi$. Informally speaking, separability of $\psi$ with respect to directions given by columns of $\mS$ is required. 
To define it formally, let us introduce first the notion of a separable set.
\begin{definition}\label{def:separable_set}
Set $Q \subseteq \R^d$ is called $D$-separable, if $\forall x, y \in Q, \mS \in D$:
\[
\mZ x + (\mI^d- \mZ)y  \in  Q.
\]
\end{definition}
Let $e\in \R^d$ be the vector of all ones. Then, for arbitrary functions, we have
\begin{definition}\label{def:separable}
Function $\phi: \R^d \rightarrow \R \cup \{ +\infty \}$ is $D$-separable if
$\dom \phi$ is $D$-separable, and there is map $\phi': \dom \phi \rightarrow \R^d$ such that
\begin{enumerate}
\item  $\forall x \in \dom\phi:\; \phi(x) = \langle \phi'(x), e \rangle$,
\item $\forall x,y \in \dom\phi, \mS\in D: \; \phi'(\mZ x + (\mI^d- \mZ)y) = \mZ\phi'(x) + (\mI^d-\mZ) \phi'(y)$.		
\end{enumerate}
\end{definition}	


\begin{example}
If $D$ is a set of matrices whose columns are standard basis vectors, $D$-separability reduces to classical (coordinate-wise) separability.
\end{example}

\begin{example}
If $D$ is set of matrices which are column-wise submatrices of orthogonal $\mU$, $D$-separability of $\phi$ reduces to classical coordinate-wise separability of $\phi(\mU^\top x)$.
\end{example}

\begin{example}
$\phi(x) = \frac12\| x\|^2$ is $D$-separable for any~$D$.
\end{example}

\begin{assumption}\label{as:sscn_separable}
Function $\psi$ is $\Range{\cD}$-separable.
\end{assumption}

We are now ready to present the convergence rate of {\tt SSCN}. 

\subsection{Theory}


First, let us introduce the critical lemma from which the main global complexity results are derived. Our first lemma gives a bound on the expected progress after a single step of {\tt SSCN}.

\begin{lemma}\label{lem:sscn_keylemma}
Let Assumptions~\ref{as:sscn_conv_lipschitz},~\ref{as:sscn_uniform},~\ref{as:sscn_smooth} and~\ref{as:sscn_separable} hold.
Then, for every $k \geq 0$ and $y \in \R^d$ we have
\begin{equation} \label{GlobalUpper}
 \E{F(x^{k + 1}) \, | \, x^k } 
 \leq 
\left( 1 - \frac{\tau}{d} \right) F(x^k) + \frac{\tau}{d} F(y)   + \frac{\tau}{d} \left(  \frac{d - \tau}{d } \frac{L}{2}\|y - x^k\|^2 + \frac{M}{3}\|y - x^k\|^3
\right).
\end{equation}
\end{lemma}

Now we are ready to present global complexity results for the general class of convex functions. The convergence rate is obtained by summing ~\eqref{GlobalUpper} over the different iterations $k$, and with a specific choice of $y$. 

\begin{theorem}\label{thm:sscn_global_weakly}
	Let Assumptions~\ref{as:sscn_conv_lipschitz},~\ref{as:sscn_uniform},~\ref{as:sscn_smooth} and~\ref{as:sscn_separable} hold. Denote
	\beq \label{Rdef}
	R  \Def  \sup\limits_{x \in \R^d} \Bigl\{  \|x - x^{*} \| \; : \; F(x) \leq F(x^{0})  \Bigr\},
	\eeq
	and suppose that $R < +\infty$.
	Then, for every $k \geq 1$ we have
	\beq \label{GlobalConv}
	  \E{ F(x^k) } - F^{*} \leq 
	\frac{d - \tau}{\tau} \cdot \frac{4.5 L R^2}{ k } + \left(\frac{d}{\tau}\right)^2 \cdot \frac{9 M R^3}{k^2}
	+ \frac{F(x^0) - F^{*}}{1 + \frac{1}{4}\left( \frac{\tau}{d} k \right)^{3}}.
	\eeq
	
\end{theorem}


Note that convergence rate of the minibatch version\footnote{Sampling $\tau$ coordinates at a time for objectives with $L$-Lipschitz gradients.} of first-order {\tt CD} is $\cO\bigl( \frac{d}{\tau} \frac{LR^2}{k}\bigr)$. At the same time, (global) convergence rate of cubically regularized Newton method is $\cO\bigl( \frac{MR^3}{k^2}\bigr)$. Therefore, Theorem~\ref{thm:sscn_global_weakly} shows that the global rate of {\tt SSCN} well interpolates between the two extremes,
depending on the sample size $\tau$ we choose.

\begin{remark}
According to estimate~\eqref{GlobalConv}, in order to have $\E{F(x^k)} - F^{*} \leq \varepsilon$,
it is enough to perform
$$
k = \cO\left(  \frac{d - \tau}{\tau} \frac{LR^2}{\varepsilon} + \frac{d}{\tau} \sqrt{\frac{MR^3}{\varepsilon}}
+ \frac{d}{\tau}\left( \frac{F(x^0) - F^{*}}{\varepsilon} \right)^{1/3}  \right)
$$
iterations of {\tt SSCN}.
\end{remark}

Next, we move to the strongly convex case.  

\begin{assumption}\label{as:sscn_sc}
Function $f$ is $\mu$-strongly convex, i.e. $\nabla^2 f(x) \succeq \mu \mI^d$ for all $x\in \R^d$.
\end{assumption}

\begin{remark}
Strong convexity of the objective (assumed for Theorem~\ref{thm:sscn_global_strongly} later) implies:
$ R < +\infty$. Furthermore, due to monotonicity of the sequence $\{ F(x_k) \}_{k \geq 0}$ (see Remark~\ref{rem:monotonic}), we have
$\|x^k - x^{*}\| \leq R$ for all $k$. Therefore, it is sufficient to require Lipschitzness of gradients over the sublevel set, which holds with $L = \lambda_{\max}(\nabla^2 f(x^{*})) + MR$.
\end{remark}


As both extremes cubic regularized Newton (where $\mS = \mI^d$ always) and (first-order) {\tt CD} ($\mS = e_i$ for randomly chosen $i$) enjoy (global) linear rate under strong convexity, linear convergence of {\tt SSCN} is expected as well. At the same time, the leading complexity term should be in between the two extremes. Such a result is established as Theorem~\ref{thm:sscn_global_strongly}.

\begin{theorem}\label{thm:sscn_global_strongly}
Let Assumptions~\ref{as:sscn_conv_lipschitz},~\ref{as:sscn_uniform},~\ref{as:sscn_separable}
and~\ref{as:sscn_sc} hold. 
Then, 
$ \E{F(x^k)} - F^{*} \leq  \varepsilon$,
as long as the number of iterations of {\tt SSCN} is
$$
 k =   \cO\left( \left(  \frac{d - \tau}{\tau} \frac{L}{\mu} + \frac{d}{\tau}\sqrt{\frac{M R}{\mu}} + \frac{d}{\tau}     
\right) 
\cdot \log \frac{F(x^0) - F^{*}}{\varepsilon}  \right) .
$$
\end{theorem}

Indeed, if $\mS =\mI^d$ with probability 1 and $MR\geq \mu$, the leading complexity term becomes $\sqrt{\frac{MR}{\mu}} \log\frac{1}{\varepsilon}$ which corresponds to the global complexity of cubically regularized Newton for
minimizing strongly convex functions~\cite{nesterov2006cubic}.
On the other side of the spectrum if $\mS = e_i$ with probability $\frac1d$, the leading complexity term becomes $\frac{dL}{\mu} \log\frac{1}{\varepsilon}$, which again corresponds to convergence rate of {\tt CD}~\cite{rcdm}. 
Lastly, if $1<\tau<d$, the global linear rate interpolates the rates mentioned above.

\begin{remark}
Proof of Theorem~\ref{thm:sscn_global_strongly} only uses the following consequence of strong convexity:
\beq \label{eq:sscn_SConvex}
\frac{\mu}{2}\|x - x^{*}\|^2  \leq F(x) - F^{*}, \qquad x \in \R^d
\eeq
and thus the conditions of Theorem~\ref{thm:sscn_global_strongly} might be slightly relaxed.\footnote{However, this relaxation is not sufficient to obtain the local convergence results.} For detailed comparison of various relaxations of strong convexity, see~\cite{karimi2016linear}.
\end{remark}


\section{Local convergence \label{sec:sscn_local}}

Throughout this section, assume that $\psi = 0$. We first present the key descent lemma, which will be used to obtain local rates. Let $\mH_{\mS}(x) \eqdef  \nabla^2_{\mS} f(x) +\sqrt{ \frac{M_{\mS}}{2}} \| \nabla_{\mS} f(x)\|^{\frac12} \mI^{\tau(\mS)} $.

\begin{lemma} \label{lem:sscn_decrease}
\begin{equation}\label{eq:sscn_decrease}
f(x^k)-f(x^{k+1})  \geq   \frac12 \| \nabla_{\mS} f(x^k)\|^2_{  \mH^{-1}(x^k)  }.
\end{equation}
\end{lemma}



Before stating the convergence theorem, it will be suitable to define the stochastic condition number of  $\mH_*\eqdef \nabla^2 f(x^*)$:
\begin{equation}\label{eq:sscn_sc_generalized}
\zeta  \eqdef \lambda_{\min} \left( \mH_*^{\frac12}  \E{{\mS} \left(\mS^\top \mH_* \mS \right)^{-1}{\mS}^\top}  \mH_*^{\frac12} \right),
\end{equation}
as it will drive the local convergence rate of {\tt SSCN}. 


\begin{theorem}[Local Convergence]\label{thm:sscn_local}
Let Assumptions~\ref{as:sscn_conv_lipschitz},~\ref{as:sscn_sc} hold, and suppose that $\psi = 0$. 
 For any $\varepsilon>0$ there exists $\delta>0$ such that if $F(x^0) - F^* \leq \delta$, we have
\begin{equation}\label{eq:sscn_local_rate}
\E{F(x^k) - F^*} \leq \left( 1- (1-\varepsilon)\zeta  \right)^k\left( F(x^0) - F^*\right)
\end{equation}
and therefore the local complexity of {\tt SSCN} is $\cO\left( \zeta^{-1} \log\frac1\varepsilon\right)$. If further $M=0$ (i.e. $f$ is quadratic), then $\varepsilon =0$ and $\delta = \infty $, and thus the rate is global.


\end{theorem} 


The proof of Theorem~\ref{thm:sscn_local} along with the exact formulas for $\varepsilon,\delta$ can be found in Section~\ref{sec:sscn_local_proofs} of the Appendix. 


Theorem~\ref{thm:sscn_local} provides a local linear convergence rate of {\tt SSCN}. While one might expect a superlinear rate to be achievable, this is not the case, and we argue that the rate from Theorem~\ref{thm:sscn_local} is the best one can hope for. 

In particular, if $M = 0$, Algorithm~\ref{alg:sscn_crcd} becomes subspace descent for minimizing positive definite quadratic which is a specific instance of sketch-and-project~\cite{gower2015randomized}. However, sketch-and-project only converges linearly -- the iteration complexity of sketch-and-project to minimize $(x-x^*)^\top \mA (x-x^*)$ with $\mA\succ 0$ is 
\[ \cO\left( \left( \mA^{\frac12}  \E{{\mS}\left( \mS^\top \mA \mS \right)^{-1}{\mS}^\top}  \mA^{\frac12} \right)^{-1}\log\frac1\varepsilon\right). \]
 Notice that this rate is matched by Theorem~\ref{thm:sscn_local} in this case. 


Next, we compare the local rate of {\tt SSCN} to the rate of {\tt SDNA}~\cite{sdna}. To best of our knowledge, {\tt SDNA} requires the least oracle calls to minimize $f$ among all first-order non-accelerated methods.


\begin{remark}
{\tt SDNA} is a first-order analogue to Algorithm~\ref{alg:sscn_crcd} with $\mS=\mI^d_{(:,S)}$. In particular, given matrix $\mL$ such that $\mL\succeq \nabla^2 f(x) \succ 0 $ for all $x$, the update rule of {\tt SDNA} is $$x^+ = x - \mS \left( \mS^\top \mL \mS \right)^{-1} \nabla_{\mS} f(x),$$ where $\mS = \mI^d_{(:,S)}$ for a random subset of columns $S$.  {\tt SDNA} enjoys linear convergence rate with leading complexity term $\left(\mu \lambda_{\min} \left(\E{\mS(\mS^\top \mL \mS)^{-1}\mS^\top} \right)\right)^{-1}$. The leading complexity term of {\tt SSCN} is $\zeta^{-1}$, and we can bound
\begin{eqnarray*}
\zeta &\geq & \lambda_{\min}\left( \mH_* \right) \lambda_{\min} \left(\E{{\mS} \left(\mS^\top \mH_* \mS\right)^{-1}{\mS}^\top}   \right)
\\
& \geq & \mu \lambda_{\min} \left(\E{\mS \left( \mS^\top \mL \mS \right)^{-1}\mS^\top}\right).
\end{eqnarray*}
Hence, the local rate of {\tt SSCN} is no worse than the  rate of {\tt SDNA}. Furthermore, both of the above inequalities might be very loose in some cases (i.e., there are examples where $\frac{\zeta}{ \mu \lambda_{\min}\E{\mS(\mL_\mS)^{-1}\mS^\top} }$ can be arbitrarily high). Therefore, local convergence rate of {\tt SSCN} might be arbitrarily better than the convergence rate of {\tt SDNA}. As a consequence, the local convergence of {\tt SSCN} is better than convergence rate of any non-accelerated first-order method.\footnote{The rate of {\tt SSCN} and rate of accelerated subspace descent methods are not directly comparable -- while the (local) rate of {\tt SSCN} might be better than rate of ACD, the reverse might happen as well. However, both ACD and {\tt SSCN} are faster than non-accelerated subspace descent.}.
\end{remark}

Lastly, the local convergence rate provided by Theorem~\ref{thm:sscn_local} recovers the superlinear rate of cubic regularized Newton's method, as the next remark states.

 \begin{remark}
 If $\mS = \mI^d$ with probability 1, Algorithm~\ref{alg:sscn_crcd} becomes cubic regularized Newton method~\cite{griewank1981modification, nesterov2006cubic}. For $\mH_*\eqdef \nabla^2 f(x^*)$ we have 
 \begin{align*}
 \zeta = \lambda_{\min} \left( \mH_*^{\frac12} \mH_*^{-1} \mH_*^{\frac12} \right) =  \lambda_{\min} (\mI^d) = 1.
 \end{align*}
As a consequence of Theorem~\ref{thm:sscn_local}, for any $\varepsilon>0$ there exists $\delta>0$ such that if $F(x)-F(x^*)\leq \delta$, we have
 \[
 F(x^+)- F(x^*)\leq \varepsilon(F(x)-F(x^*)).
 \]
 Therefore, we obtain a superlinear convergence rate. 
 \end{remark}
 
 



\section{Applications}
\label{sec:sscn_applications}

\subsection{Linear models\label{sec:sscn_linear}}
Consider only $\mS = \mI^d_{(:,S)}$ for simplicity.
 Let 
 \begin{equation} \label{eq:sscn_linear_model}
  F(x) \eqdef \frac1n \sum \limits_{i=1}^n \phi_i( \la a_i, x \ra )+ \psi(x),
 \end{equation}
 and $f(x) \eqdef \frac1n \sum_{i=1}^n \phi_i( \la a_i, x \ra )$ 
  and suppose that $|\nabla^3 \phi_i (y)| \leq c$. Then clearly, for any $h \in \R^d$, we have $$\nabla^3 f(x)[h]^3 =\frac1n \sum_{i=1}^n \nabla^3\phi_i( \la a_i, x\ra ) \la a_i, h \ra^3 .$$ While evaluating \[E\eqdef \max_{\|h\|=1, x} \nabla^3 f(x)[h]^3 \] is infeasible, we might bound it instead via
\begin{align}
 E &\leq \max \limits_{\|h\|=1}  \frac{c}{n}\sum \limits_{i=1}^n| \la a_i, h \ra |^3  \leq    \frac{c}{n}\sum \limits_{i=1}^n\|a_i\|^3, \label{eq:sscn_ndanjdajn}
\end{align}
which means that $M=\frac{c}{n} \sum_{i=1}^n \| a_i\|^3$ is a feasible choice. On the other hand, for $S = \{ j \}$ we have
 \[
\max \limits_{\|h_j\|=1, x} \nabla^3 f(x)[h_j]^3 = \max \limits_{x} \nabla^3 f(x)[e_j]^3 \leq \frac{c}{n} \sum \limits_{i=1}^n|a_{ij}|^3 
 \]
 and thus we might set $M_j =\frac{c}{n} \sum_{i=1}^n | a_{ij}|^3$. The next lemma compares the above choices of $M$ and $M_j$.

\begin{lemma}
We have $M\geq \max_j M_j$. At the same time, there exist vectors $a_i$ that $\max_j M_j  = \frac{M}{d^{\frac32}}$.
\end{lemma}
\begin{proof}
The first part is trivial. For the second part, consider $a_{i,j}\in \{-1,1\}$. 
\end{proof}

\begin{remark}
One might avoid the last inequality from~\eqref{eq:sscn_ndanjdajn} using polynomial optimization; however, this might be more expensive than solving the original optimization problem and thus is not preferable. Another strategy would be to use a line search, see Section~\ref{sec:sscn_solving}.
\end{remark}

Both the formula for $M$ and the formula for $M_j$ require the prior knowledge of $c\geq 0$ such that $|\nabla^3 \phi_i (y)| \leq c$ for all $i$. The next Lemma shows how to compute such $c$ for the logistic regression (binary classification model).

\begin{lemma}
Let $\phi_i(y) = \log(1+e^{-b_iy}),  b_i \in \{-1,1\}$. Then $c = \frac{1}{6\sqrt{3}}$.
\end{lemma}
\begin{proof}
$\nabla^3 \phi_i(y) = -\frac{e^x(e^x-1)}{(1+e^x)^3}$ $\Rightarrow$ $\left| \nabla^3 \phi_i(y) \right|\leq \frac{1}{6\sqrt{3}}$.
\end{proof}

\paragraph{Cost of performing a single iteration}
For the sake of simplicity, let $\tau(\mS)=1$, $\psi\equiv0$. Any {\tt CD} method (i.e. method with update rule~\eqref{eq:sscn_update_general} with $\mS\in \{e_1, \dots, e_d\}$) can be efficiently implemented by memorizing the residuals $\la a_i, x^k \ra$, which is cheap to track since $x^{k+1} - x^k$ is a sparse vector. The overall cost of updating the residuals is $\cO(n)$ while the cost of computing $\nabla_i f(x)$ and $\nabla^2_{i,i} f(x)$ (given the residuals are stored) is $\cO(n)$. Therefore the overall cost of performing a single iteration is $\cO(n)$. Generalizing to $\tau(\mS)=\tau\geq 1$, the overall cost of single iteration of {\tt SSCN} can be estimated as $\cO(n\tau^2 + \tau^3)$,
where $\cO(n\tau^2)$ comes from evaluating subspace gradient and Hessian, while $\cO(\tau^3)$ comes from solving the cubic subproblem.



\subsection{Dual of linear models \label{sec:sscn_dual}}
So far, all results and applications for {\tt SSCN} we mentioned were problems with large model size $d$. In this section we describe how {\tt SSCN} can be efficient to tackle big data problems in some settings. Let $\mA\in \R^{n\times d}$ is data matrix and consider a specific instance of~\eqref{eq:sscn_linear_model} where
\begin{equation}\label{eq:sscn_to_be_dualized}
\ \min_{x\in \R^d} \left\{ F_P(x) \eqdef  \frac1d \sum \limits_{i=1}^n \rho_i(\mA_{(:,i)}x) + \frac{\lambda}{2} \|x \|^2 \right\}.
\end{equation}
where $\rho_i$ is convex for all $i$. One can now formulate a dual problem of~\eqref{eq:sscn_to_be_dualized} as follows:
\begin{equation}\label{eq:sscn_dual_linear}
 \max_{y\in \R^n} \left\{ F_D(y) \eqdef - \frac{1}{2\lambda n^2} \left\| \mA^\top y \right\|^2 -\frac{1}{n} \sum \limits_{i=1}^n\rho_i^*(e_i^\top x) \right\}.
\end{equation}
Note that~\eqref{eq:sscn_dual_linear} is of form~\eqref{eq:sscn_linear_model}, and therefore if $\rho^*_i$ has Lipschitz Hessian, we can apply {\tt SSCN} to efficiently solve it (same as Section~\ref{sec:sscn_linear}). Given the solution of~\eqref{eq:sscn_dual_linear}, we can recover the solution of~\eqref{eq:sscn_to_be_dualized} (duality theory). Thus, {\tt SSCN} can be used as a data-stochastic method to solve finite-sum optimization problems.

The trick described in this section is rather well known. It was  first used in~\cite{sdca}, where  {\tt CD} applied to the problem~\eqref{eq:sscn_dual_linear} ({\tt SDCA}) was shown to be competitive with the variance reduced methods like {\tt  SAG}~\cite{sag}, {\tt SVRG}~\cite{svrg} or {\tt SAGA}~\cite{saga}.

%\subsection{Zero-order optimization \label{sec:sscn_zero}}
%Our method is applicable in the setup where function $f$ is accessible via zeroth-order oracle only. In such case, for any $\mS \in \R^{\tau\times d}$ we can estimate $\nabla_{\mS} f(x)$ and $ \nabla_\mS^2 f(x)$ using $\cO(\tau^2)$ function value evaluations. However, since both $\nabla_{\mS} f(x)$ and $ \nabla_\mS^2 f(x)$ are only evaluated inexactly, a slight modification of our theory would be required. 









\section{Experiments}
We now numerically verify our theoretical claims. We consider two different objectives: logistic regression (Section~\ref{sec:logreg}) and log-sum-exp (Section~\ref{sec:logsumexp}).






\subsection{Logistic regression\label{sec:logreg}}
Regularized logistic regression is a machine learning model for binary classification. Given data matrix $\mA\in \R^{n\times d}$, labels $b\in \{-1, 1\}^{n}$ and regularization parameter $\lambda \in \R_{+}$, the training corresponds to solving the following optimization problem
\[
f(x)= \frac1n \sum_{i=1}^n \log \left(1+\exp\left(\mA_{i,:}x\cdot  b_i\right) \right)+\frac{\lambda}{2} \| x\|^2.
\]

In the first experiment, we compare {\tt SSCN} to first-order coordinate descent ({\tt CD}) on LIBSVM~\cite{chang2011libsvm}. We consider three different instances of {\tt CD}: {\tt CD} with uniform sampling, {\tt CD} with importance sampling~\cite{rcdm}, and accelerated {\tt CD} with importance sampling~\cite{allen2016even, nesterov2017efficiency}. 

In order to be comparable with the mentioned first-order methods, we consider $\mS\in \{e_1, \dots, e_d\}$ with probability 1  -- the complexity of performing each iteration is about the same for each algorithm now. At the same time, computing $M_{e_i}$ for all $1\leq i \leq d$ is of cost $\cO(nd)$ -- the same cost as computing coordinate-wise smoothness constants for (accelerated) {\tt CD} (see Section~\ref{sec:sscn_linear} for the details). Figure~\ref{fig:sscn_libsvm} shows the result for non-normalized data, while Figure~\ref{fig:sscn_libsvm_normalzied} shows the results for normalized data (thus importance sampling is identical to uniform). 

In all examples, {\tt SSCN} outperformed {\tt CD} with uniform sampling. Moreover, the performance of {\tt SSCN} was always either about the same or significantly better to {\tt CD} with importance sampling. Furthermore, {\tt SSCN} was also competitive to accelerated {\tt CD} with importance sampling (in about half of the cases, {\tt SSCN} was better, while in the other half, ACD was better).



\begin{figure}[!h]
\centering
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDatasetw1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDataseta1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDatasetmushrooms.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDatasetphishing.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDatasetmadelon.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDatasetduke.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDatasetgisette_scale.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDataseta9a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochDatasetw8a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\caption{Comparison of {\tt CD} with uniform sampling, {\tt CD} with importance sampling, accelerated {\tt CD} with importance sampling and {\tt SSCN} (Algorithm~\ref{alg:sscn_crcd}) with uniform sampling on LibSVM datasets.} 
\label{fig:sscn_libsvm}
\end{figure}


\begin{figure}[!h]
\centering
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDatasetw1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDataseta1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDatasetmushrooms.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDatasetphishing.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDatasetmadelon.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDatasetduke.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDatasetgisette_scale.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDataseta9a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{CRCDvsCDepochnormDatasetw8a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\caption{Comparison of coordinate descent, accelerated coordinate descent and {\tt SSCN} (all with uniform sampling) on LibSVM datasets. In each case we have normalized the data matrix to have identical norms of all columns.} 
\label{fig:sscn_libsvm_normalzied}
\end{figure}



In the second experiment, we compare methods with $\tau>1$: {\tt SSCN} and {\tt SDNA}~\cite{sdna} (analogous first-order method). Again, we consider the logistic regression problem on LIBSVM data. We consider $\tau \in \{1,5,25\}$. In all cases, we sample uniformly --  every subset of size $\tau$ have equal chance to be chosen at every iteration (independent of the past). 

There is, however, one tricky part in terms of implementation. While we can evaluate and store $M_{e_i}$ ($i\leq d$) cheaply for linear models, this is not the case for evaluating/storing $M_S$ (at least we do not know how to do it efficiently). Therefore, we use $M_S = M$ for $|S|>1$ for {\tt SSCN}. Figure~\ref{fig:sscn_libsvm_sdna} shows the result. As expected, {\tt SSCN} has outperformed {\tt SDNA}. 
 
 

\begin{figure}[!h]
\centering
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDatasetw1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDataseta1a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDatasetmushrooms.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDatasetphishing.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDatasetmadelon.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDatasetduke.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\\
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDatasetgisette_scale.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDataseta9a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width =  \textwidth ]{SDNAepochDatasetw8a.pdf}
        %\caption{ Residual vs. iteration  }\label{fig:sscn_bl_ex_flops}
\end{minipage}%
\caption{{\tt SSCN} vs. {\tt SDNA} on LibSVM datasets. All algorithms with uniform sampling.} 
\label{fig:sscn_libsvm_sdna}
\end{figure}


\subsection{Log-sum-exp \label{sec:logsumexp}}

In this section, let us consider unconstrained minimization of the following Log-sum-exp function
$$
f(x)  =  \sigma \log\left( \sum\limits_{i = 1}^m \exp \left( \frac{\la a_i, x \ra - b_i}{\sigma} \right) \right),
\quad x \in \R^d,
$$
where $\sigma > 0$ is a \textit{smoothing} parameter, while
$a_i \in \R^n, 1 \leq i \leq m$ and $b \in \R^m$ are given data.
This function has both Lipschitz continuous gradient and Lipschitz continuous Hessian
(see Example~1 in~\cite{doikov2019minimizing}). 

In our experiments, we first generate randomly elements of $\{ \tilde{a}_i \}_{i = 1}^m$ and $b$ from
uniform distribution on $[-1, 1]$. Then, we form an auxiliary function 
\[\tilde{f}(x) \eqdef \sigma \log\left( \sum\limits_{i = 1}^m \exp \bigl(  \frac{\la \tilde{a}_i, x \ra - b_i}{\sigma} \bigr) \right),\]
using these parameters, and set
$$
a_i   \eqdef  \tilde{a}_i - \nabla \tilde{f}(0), \quad 1 \leq i \leq m.
$$
Thus, we essentially obtain the optimum $x^{*}$ of $f$ in the origin, since $\nabla f(0) = 0$.
We use $x_0 \eqdef e$ (vector of all ones) as a starting point,
and always set $m  \eqdef 6d$.

For this problem, we compare the performance of {\tt SSCN} with the first-order Coordinate Descent ({\tt CD}), using uniform samples of coordinates $S \subseteq [d]$ of a fixed size $\tau = |S|$. 

Note, that keeping scalar products $\{ \la a_i, x_k \ra \}_{i = 1}^m$
precomputed for a current point $x_k$, we are able to compute the partial gradient
$\nabla_{\mS} f(x^k)$ in time $O(\tau m)$ and the partial Hessian $\nabla^2_{\mS} f(x^k)$ in time $O(\tau^2 m)$.
To find the next direction $h^k$ of {\tt SSCN} (solving the Cubic subproblem), we call Nonlinear Conjugate Gradient method,
and use the following condition as a stopping criterion:
$$
\| \nabla_h T_{\mS}(x^k; h^k) \|  \leq  10^{-4},
$$
where $T_{\mS}(x^k; h)   \eqdef \la \nabla_{\mS} f(x^k), h \ra + \frac{1}{2}\la \nabla_{\mS}^2 f(x^k)h, h \ra + \frac{M_k}{6}\|\mS h\|^3$ is the Cubic model, and $M_k \geq 0$ is a regularization constant.

For both methods, we use one-dimensional search at every iteration, to fit the corresponding parameter:
\begin{enumerate}
	\item For the Coordinate Descent, we find $L_k$ such that $f(x^{k}) - f(x^{k + 1}) \geq \frac{1}{2L_k}\| \nabla_{\mS} f(x^k) \|^2$, 
	where $x^{k + 1}$ is the next point of the method: $x^{k + 1} = x^k + \frac{1}{L_k}\mS \nabla_{\mS} f(x^k)$.
	
	\item For {\tt SSCN}, we find $M_k$ such that~\eqref{eq:sscn_coordinate_ub_full}
	is satisfied, i.e. $f(x^{k}) - f(x^{k + 1}) \geq -T_{\mS}(x^k, h^k)$.
\end{enumerate}
Therefore,  we need to evaluate the function value inside the procedure, which is not very expensive.


The results are shown on Figures~\ref{fig:sscn_log_sum_exp_500},\ref{fig:sscn_log_sum_exp_1000},
for $d = 500$ and $1000$ respectively\footnote{Clock time was evaluated using the machine with Intel Core i7-8700 CPU, 3.20GHz; 16 GB RAM.}.
We see, that {\tt SSCN} outperforms {\tt CD} significantly in terms of the iteration rate.
For {\tt SSCN} with a medium batchsize $\tau$, we may obtain the best performance 
in terms of the total computational time.

\begin{figure}[h!]
	\centering
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_500_10_iters.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_500_10_time.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_500_10_iters.pdf}
	\end{minipage}
	\\
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_500_10_time.pdf}
	\end{minipage}
		\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_500_05_iters.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_500_05_time.pdf}
	\end{minipage}
	\\
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_500_05_iters.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_500_05_time.pdf}
	\end{minipage}
	
	
	\caption{{\tt SSCN} and Coordinate Descent ({\tt CD}) methods, minimizing Log-Sum-Exp function, $d = 500$.} 
	\label{fig:sscn_log_sum_exp_500}
\end{figure}



\begin{figure}[h!]
	\centering
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_1000_10_iters.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_1000_10_time.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_1000_10_iters.pdf}
	\end{minipage}
	\\
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_1000_10_time.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_1000_05_iters.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_CD_1000_05_time.pdf}
	\end{minipage}
	\\
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_1000_05_iters.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width =  \textwidth ]{logsumexp_SSCN_1000_05_time.pdf}
	\end{minipage}
	
	
	\caption{{\tt SSCN} and Coordinate Descent ({\tt CD}) methods, minimizing Log-Sum-Exp function, $d = 1000$.} 
	\label{fig:sscn_log_sum_exp_1000}
\end{figure}




\section{Conclusion}

In this chapter, we have introduced {\acrshort{SSCN}}, which is both a subspace version cubically-regularized Newton method~\cite{nesterov2006cubic}, and a second-order enhancement of stochastic subspace descent~\cite{kozak2019stochastic}. The algorithm enjoys the global convergence to the optimum along with the fast local rates. We believe our method opens up several new avenues for the future research which we list next.

\paragraph{Acceleration.} We believe it would be valuable to incorporate Nesterov's momentum into Algorithm~\ref{alg:sscn_crcd}. Ideally, one would like to get the global rate in between convergence rate of accelerated cubic regularized Newton~\cite{nesterov2008accelerating} and accelerated {\tt CD}~\cite{allen2016even, nesterov2017efficiency}. On the other hand, the local rate (for strongly convex objectives) should recover accelerated sketch-and-project~\cite{tu2017breaking, gower2018accelerated}. If accelerated sketch-and-project is optimal (this is yet to be established), then accelerated {\tt SSCN} (again, given that it recovers accelerated sketch-and-project) would be a locally optimal algorithm as well.

\paragraph{Non-separable $\psi$.} As mentioned in Section~\ref{sec:sscn_setup}, one should not hope for linear convergence of {\tt SSCN} if $\psi$ is not separable, as the iterates can ``jump'' away from the optimum in such case. This issue has been resolved for first-order methods using control variates in Chapter~\ref{sega} via {\tt SEGA} algorithm. Therefore, the development of second-order {\tt SEGA} remains an interesting open problem.


\paragraph{Inexact method.} {\tt SSCN} is applicable in the setup, where function $f$ is accessible via zeroth-order oracle only. In such a case, for any $\mS \in \R^{\tau\times d}$ we can estimate $\nabla_{\mS} f(x)$ and $ \nabla_\mS^2 f(x)$ using $\cO(\tau^2)$ function value evaluations. However, since both $\nabla_{\mS} f(x)$ and $ \nabla_\mS^2 f(x)$ are only evaluated inexactly, a slight modification of our theory is required. 


\paragraph{Non-uniform sampling.} Note that our local theory allows for arbitrary non-uniform distribution of $\mS$, which might be potentially exploited. While developing optimal and implementable importance sampling for the local convergence is beyond the scope of this work,\footnote{As this is still an open problem even for sketch-and-project~\cite{gower2015randomized}. }
we sketch several possible sampling strategies that might yield faster convergence.\footnote{This only applies to the local results as the global convergence requires some uniformity; see Assumption~\ref{as:sscn_uniform}.} 


\begin{itemize}
\item Let $\Prob(\mS \in \{e_1, e_2, \dots, e_d \})=1$. If we evaluate the diagonal of the Hessian close to optimum (cost $\cO(nd)$ for linear models) and sample proportionally to it, we obtain local linear rate with leading complexity term $\frac{\Tr{\nabla^2 f(x^*)}}{\lambda_{\min}\nabla^2 f(x^*)}$. 

\item It is unclear how to design an efficient importance sampling for minibatch (i.e. $1<\E{\tau(\mS)}<d$) methods. Determinantal point processes (DPP)~\cite{rodomanov2019randomized, mutny2019convergence} were proposed to speed up {\tt SDNA} from~\cite{sdna} (i.e., analogous {\tt CD} with static matrix upper bound) -- we thus believe they might be applicable on our setting too. However, in such a case, one would need to evaluate the whole Hessian close to optimum, which is infeasible for applications where $d$ is large.

\item It is known that {\tt SDNA} (see related literature) is faster than minibatch {\tt CD} under the ESO assumption~\cite{qu2016coordinate1, qu2016coordinate2}. Therefore, we might instead apply minibatch importance sampling for ESO assumption from~\cite{hanzely2018accelerated} (which corresponds to optimizing the upper bound on iteration complexity). Using the mentioned sampling, we only require evaluating the diagonal of Hessian at some point close to optimum, which is of the same cost as computing the full gradient for linear models -- thus is feasible.

\item It is a natural question to ask whether one can speed up the convergence using greedy rule instead of random one. For standard {\tt CD}, greedy rule was shown to have a superior iteration complexity to any randomized rule~\cite{nutini2015coordinate, karimireddy2018efficient}. For simplicity, consider case where $\Prob(\mS \in \{e_1, e_2, \dots, e_d \})=1$. Far from the optimum, (approximate) greedy rule at iteration $k$ chooses index $i = \argmax_{j} | \nabla_j f(x^k)|^{\frac32}M_{e_j}^{-\frac12}$. Close to optimum, if a diagonal of a Hessian was evaluated, (approximate) greedy index would be $\argmax_{j} | \nabla_j f(x^k)|^{2}\nabla_{j,j} f(x)^{-1}$. For linear models, both of the mentioned cases are implementable using the efficient neirest neighbour search~\cite{dhillon2011nearest} with sublinear complexity in terms of $d$.

\end{itemize}
 

